Continuous Adjoint Complement to the Blasius Equation

The manuscript is concerned with a continuous adjoint complement to two-dimensional, incompressible, first-order boundary-layer equations for a flat plate boundary-layer. The text is structured into three parts. The first part demonstrates, that the adjoint complement can be derived in two ways, either following a first simplify then derive or a first derive and then simplify strategy. The simplification step comprises the classical boundary-layer (b.-l.) approximation and the derivation step transfers the primal flow equation into a companion adjoint equation. The second part of the paper comprises the analyses of the coupled primal/adjoint b.-l. framework. This leads to similarity parameters, which turn the Partial-Differential-Equation (PDE) problem into a boundary value problem described by a set of Ordinary-Differential-Equations (ODE) and support the formulation of an adjoint complement to the classical Blasius equation. Opposite to the primal Blasius equation, its adjoint complement consists of two ODEs which can be simplified depending on the treatment of advection. It is shown, that the advective fluxes, which are frequently debated in the literature, vanish for the investigated self-similar b.l. flows. Differences between the primal and the adjoint Blasius framework are discussed against numerical solutions, and analytical expressions are derived for the adjoint b.-l. thickness, wall shear stress and subordinated skin friction and drag coefficients. The analysis also provides an analytical expression for the shape sensitivity to shear driven drag objectives. The third part assesses the predictive agreement between the different Blasius solutions and numerical results for Navier-Stokes simulations of a flat plate b.-l. at Reynolds numbers between 1E+03 <= ReL <= 1E+05 .

==> tex/blasius_derivations.tex <==
\section{Blasius Derivation Area}

\subsection{Seeking for Primal Similarity Variables}
Integrating the primal boundary layer Equ. \ref{equ:primal_bounday_layer_mome1_first} along the $y$ ($x_\mathrm{2}$) direction and neglecting the pressure gradient yields:
\begin{align}
\int_0^\delta u  \frac{\partial u}{\partial x} \mathrm{d} y 
+ \int_0^\delta v \frac{\partial u}{\partial y} \mathrm{d} y 
- \int_0^\delta \nu \frac{\partial^2 u}{\partial y^2} \mathrm{d} y  = 0.
\end{align}
Integration by parts of the second term offers:
\begin{align}
\int_0^\delta u \frac{\partial u}{\partial x} \mathrm{d} y 
+ \left[u v \right]_0^y
- \int_0^\delta \frac{\partial v}{\partial y} u \mathrm{d} y 
- \int_0^\delta \nu \frac{\partial^2 u}{\partial y^2} \mathrm{d} y  = 0.
\end{align}
Continuity Equ. \ref{equ:primal_bounday_layer_mass1_first} offers a link between $u$ and $v$:
\begin{align}
\frac{\partial v}{\partial y} = - \frac{\partial u}{\partial x} \hspace{1cm} \Rightarrow \hspace{1cm} v(y) = - \int_0^y \frac{\partial u}{\partial x} \mathrm{d} y .
\end{align}
Considering no slip along $y=0$, we end up with an expression independent of v:
\begin{align}
\int_0^\delta u \frac{\partial u}{\partial x} \mathrm{d} y 
- u  \int_0^\delta \frac{\partial u}{\partial x} \mathrm{d} y 
+ \int_0^\delta \frac{\partial u}{\partial x} u \mathrm{d} y 
- \nu \frac{\partial u}{\partial y}\bigg|_0^\delta  = 0.
\end{align}
Trying to express the main flow velocity by:
\begin{align}
\frac{u}{u_\infty} = g \bigg( \underbrace{\frac{y}{\delta (x)}}_{\eta} \bigg)
\end{align}
where $g$ is a function of $\eta = y / \delta (x)$ only, we end up with its spatial derivatives:
\begin{align}
u &= u_\infty g \\
\frac{\partial u}{\partial x} &= - u_\infty g^\prime \frac{y}{\delta^2} \frac{\partial \delta}{\partial x} \\
\frac{\partial u}{\partial y} &= u_\infty g^\prime \frac{1}{\delta}.
\end{align}
Substituting them yields:
\begin{align}
-2 u_\infty^2 \int_0^\delta  g g^\prime \frac{y}{\delta^2} \frac{\partial \delta}{\partial x} \mathrm{d} y 
+ u_\infty^2  \int_0^\delta  g^\prime \frac{y}{\delta^2} \frac{\partial \delta}{\partial x} \mathrm{d} y 
- \nu u_\infty g^\prime \frac{1}{\delta} \bigg|_0^\delta  = 0.
\end{align}
Substitution of $\eta = y / \delta$ ($\mathrm{dy} = \delta \mathrm{d} \eta = \delta  \mathrm{d} (y / \delta)$) offers:
\begin{align}
-2 u_\infty^2 \int_0^1  g g^\prime \frac{y}{\delta} \frac{\partial \delta}{\partial x} \mathrm{d} (\frac{y}{\delta}) 
+ u_\infty^2  \int_0^1  g^\prime \frac{y}{\delta} \frac{\partial \delta}{\partial x} \mathrm{d}(\frac{y}{\delta})  
- \nu u_\infty g^\prime \frac{1}{\delta} \bigg|_0^1  = 0.
\end{align}
The equation optically simplifies by rewriting to;
\begin{align}
\left[B - 2 A \right] \frac{\partial \delta}{\partial x} \delta  = \frac{\nu}{u_\infty} C \label{equ:primal_similarity_ode}
\end{align}
by introducing:
\begin{align}
A &= \int_0^1  g g^\prime \frac{y}{\delta} \mathrm{d} (\frac{y}{\delta}) = \int_0^1  g g^\prime \eta \, \mathrm{d} \eta  \\
B &= \int_0^1  g^\prime \frac{y}{\delta}  \mathrm{d}(\frac{y}{\delta}) = \int_0^1  g^\prime \eta \,  \mathrm{d} \eta \\
C &= g^\prime(1) - g^\prime(0).
\end{align}
Equ. \ref{equ:primal_similarity_ode} can be solved w.r.t. $\delta$:
\begin{align}
\delta = \sqrt{\frac{2 C}{b \left[ B - 2 A \right] }} \sqrt{ \frac{\nu \left[ a + bx \right]}{u_\infty}} 
\hspace{1cm} \Rightarrow \hspace{1cm} 
\delta \propto \sqrt{ \frac{\nu \left[a + bx \right]}{u_\infty} }.
\end{align}
Thus, the definition of our similarity variable reads:
\begin{align}
\eta = \frac{y}{\delta} = y \sqrt{\frac{u_\infty}{\nu  \left[a + bx \right]}}.
\end{align}
The classical situation corresponds to $a=0, b=1$. However, the coordinate system can placed elsewhere, e.g. $a = L, b = -1$ is also valid when measured from the (infinite long) plate end ($L \rightarrow \infty $).

\subsection{Primal Blasius Equation}
So far, it is unsure if this really simplifies the PDE into an ODE. Besides, the velocity components are not accessible so far. Thus, we take a stream function that directly satisfies the continuity Equ.
\begin{align}
u &= \frac{\partial \psi}{\partial y} \\
v &= -\frac{\partial \psi}{\partial x}.
\end{align}
The potential can be integrated from the first equation, viz.
\begin{align}
\psi &= \int_0^y u \mathrm{d} y \\
&= \int_0^y u_\infty g \mathrm{d} y  \\
&= \int_0^\eta u_\infty g  \frac{\mathrm{d} y}{\mathrm{d} \eta} \mathrm{d} \eta \\
&= \sqrt{\nu \left[a + bx \right] u_\infty} \underbrace{\int_0^\eta g  \mathrm{d} \eta}_{f(\eta)},
\end{align}
where we scramble the integral of $g$ over $\eta$ into the general function $f(\eta)$. Thus, we have a potential that depends on $x$ and $\eta$ only and we can compute the necessary derivatives:
\begin{align}
u &= \frac{\partial \psi}{\partial y} = \sqrt{\nu \left[ a + bx \right] u_\infty} f^\prime \frac{\partial \eta}{\partial y} = u_\infty f^\prime \\
v &= - \frac{\partial \psi}{\partial x} = \frac{1}{2} \sqrt{\frac{\nu b^2 u_\infty}{a + bx}} \left[ f^\prime \eta - f \right] \\
\frac{\partial u}{\partial x} &= - \frac{1}{2} u_\infty f^{\prime \prime} y \sqrt{\frac{u_\infty}{\nu \left[ a + bx \right]}} \frac{b}{a + bx} = - \frac{1}{2} \frac{ u_\infty b}{a + bx} f^{\prime \prime} \eta \\
\frac{\partial u}{\partial y} &= u_\infty f^{\prime \prime} \sqrt{\frac{u_\infty}{\nu \left[ a + bx \right]}} \\
\frac{\partial^2 u}{\partial y^2} &= u_\infty f^{\prime \prime \prime} \frac{u_\infty}{\nu \left[ a + bx \right]}.
\end{align}
Inserting them into the boundary layer equation results in:
\begin{align}
- \frac{1}{2} u_\infty f^\prime \frac{ u_\infty b}{a + bx} f^{\prime \prime} \eta
+  \frac{1}{2} \sqrt{\frac{\nu b^2 u_\infty}{a + bx}} \left[ f^\prime \eta - f \right] u_\infty f^{\prime \prime} \sqrt{\frac{u_\infty}{\nu \left[ a + bx \right]}}
- \nu u_\infty f^{\prime \prime \prime} \frac{u_\infty}{\nu \left[ a + bx \right]} &= 0 \\
%
- \frac{1}{2}  f^\prime \frac{ u_\infty^2 b}{a + bx} f^{\prime \prime} \eta
+  \frac{1}{2} \frac{b u_\infty^2}{a + bx} \left[ f^\prime \eta - f \right] f^{\prime \prime} 
-  u_\infty^2 f^{\prime \prime \prime} \frac{1}{a +bx} &= 0 \\
%
- \frac{1}{2}  f^\prime \frac{b}{a + bx} f^{\prime \prime} \eta
+  \frac{1}{2} \frac{b}{a + bx} \left[ f^\prime \eta - f \right] f^{\prime \prime} 
- f^{\prime \prime \prime} \frac{1}{a +bx} &= 0 \\
%
-  \frac{1}{2} \frac{b}{a + bx}  f  f^{\prime \prime} 
- f^{\prime \prime \prime} \frac{1}{a +bx} &= 0 \\
%
-  b f  f^{\prime \prime} 
- 2 f^{\prime \prime \prime}  &= 0 \\
\end{align}
which corresponds to the well known Blasius Equation. In line with the definition of the similarity variable we conduct:
\begin{align}
A &= \int_0^1  f^\prime f^{\prime \prime} \eta \, \mathrm{d} \eta  \\
B &= \int_0^1  f^{\prime \prime} \eta \,  \mathrm{d} \eta \\
C &= f^{\prime \prime} (1) - f^{\prime \prime}(0).
\end{align}

\subsection{Seeking for Adjoint Similarity Variables}
%(MEASURED FROM THE PLATE END AGAINST PRIMAL FLOW DIRECTION)
Integrating the primal boundary layer Equ. \ref{equ:adjoint_bounday_layer_mome1_first} along the $y$ ($x_\mathrm{2}$) direction and neglecting the adjoint pressure gradient yields:
\begin{align}
- \int_0^{\hat{\delta}} u \frac{\partial \hat{u}}{\partial x} \mathrm{d} y 
- \int_0^{\hat{\delta}} v \frac{\partial \hat{u}}{\partial y} \mathrm{d} y
+ \int_0^{\hat{\delta}} \hat{u}  \frac{\partial u}{\partial x} \mathrm{d} y 
- \int_0^{\hat{\delta}} \nu \frac{\partial^2 \hat{u}}{\partial y^2} \mathrm{d} y = 0.
\end{align}
Integration by parts of the second term offers:
\begin{align}
- \int_0^{\hat{\delta}} u \frac{\partial \hat{u}}{\partial x} \mathrm{d} y 
- \left[ v \hat{u} \right]_0^{\hat{\delta}}
+ \int_0^{\hat{\delta}} \hat{u} \frac{\partial v}{\partial y} \mathrm{d} y
+ \int_0^{\hat{\delta}} \hat{u}  \frac{\partial u}{\partial x} \mathrm{d} y 
- \int_0^{\hat{\delta}} \nu \frac{\partial^2 \hat{u}}{\partial y^2} \mathrm{d} y = 0.
\end{align}
Continuity Equ. \ref{equ:primal_bounday_layer_mass1_first} offers a link between $u$ and $v$:
\begin{align}
\frac{\partial v}{\partial y} = - \frac{\partial u}{\partial x} \hspace{1cm} \Rightarrow \hspace{1cm} v(y) = - \int_0^y \frac{\partial u}{\partial x} \mathrm{d} y
\end{align}
Considering no slip along $y=0$, we end up with an expression independent of v:
\begin{align}
- \int_0^{\hat{\delta}} u \frac{\partial \hat{u}}{\partial x} \mathrm{d} y 
+ \hat{u}_\infty \int_0^{\hat{\delta}} \frac{\partial u}{\partial x} \mathrm{d} y 
- \int_0^{\hat{\delta}} \hat{u} \frac{\partial u}{\partial x} \mathrm{d} y
+ \int_0^{\hat{\delta}}\hat{u}  \frac{\partial u}{\partial x} \mathrm{d} y 
- \nu \frac{\partial \hat{u}}{\partial y} \bigg|_0^{\hat{\delta}}  &= 0 \\
- \int_0^{\hat{\delta}} u \frac{\partial \hat{u}}{\partial x} \mathrm{d} y 
+ \hat{u}_\infty \int_0^{\hat{\delta}} \frac{\partial u}{\partial x} \mathrm{d} y 
- \nu \frac{\partial \hat{u}}{\partial y} \bigg|_0^{\hat{\delta}}  &= 0.
\end{align}
Interestingly, the advection term (RinR) is canceled. Trying to express the adjoint main flow velocity by:
\begin{align}
\frac{\hat{u}}{\hat{u}_\infty} = \hat{g} \bigg( \underbrace{\frac{y}{\hat{\delta} (x)}}_{\hat{\eta}} \bigg)
\end{align}
where $\hat{g}$ is a function of $\hat{\eta} = y / \hat{\delta} (x)$ only, we end up with its spatial derivatives:
\begin{align}
\hat{u} &= \hat{u}_\infty \hat{g} \\
\frac{\partial \hat{u}}{\partial x} &= - \hat{u}_\infty \hat{g}^\prime \frac{y}{\hat{\delta}^2} \frac{\partial \hat{\delta}}{\partial x} \\
\frac{\partial \hat{u}}{\partial y} &= \hat{u}_\infty \hat{g}^\prime \frac{1}{\hat{\delta}}.
\end{align}
Substituting them yields:
\begin{align}
\int_0^{\hat{\delta}} u_\infty g  \hat{u}_\infty \hat{g}^\prime \frac{y}{\hat{\delta}^2} \frac{\partial \hat{\delta}}{\partial x} \mathrm{d} y 
- \hat{u}_\infty \int_0^{\hat{\delta}} u_\infty g^\prime \frac{y}{\delta^2} \frac{\partial \delta}{\partial x} \mathrm{d} y 
- \nu \hat{u}_\infty \hat{g}^\prime \frac{1}{\hat{\delta}} \bigg|_0^{\hat{\delta}}  &= 0 \\
 u_\infty \hat{u}_\infty \int_0^{\hat{\delta}} g  \hat{g}^\prime \frac{y}{\hat{\delta}^2} \frac{\partial \hat{\delta}}{\partial x} \mathrm{d} y 
- \hat{u}_\infty u_\infty \int_0^{\hat{\delta}} g^\prime \frac{y}{\delta^2} \frac{\partial \delta}{\partial x} \mathrm{d} y 
- \nu \hat{u}_\infty \hat{g}^\prime \frac{1}{\hat{\delta}} \bigg|_0^{\hat{\delta}}  &= 0.
\end{align}
Substitution of  $\hat{\eta} = y / \hat{\delta}$ ($\mathrm{dy} = \hat{\delta} \mathrm{d} \hat{\eta} = \mathrm{d} (y / \hat{\delta})$) offers:
\begin{align}
 u_\infty \hat{u}_\infty \int_0^1 g  \hat{g}^\prime \frac{y}{\hat{\delta}} \frac{\partial \hat{\delta}}{\partial x} \mathrm{d} (\frac{y}{\hat{\delta}}) 
- \hat{u}_\infty u_\infty \int_0^1 g^\prime \frac{y}{\hat{\delta}} \frac{\hat{\delta}^2}{\delta^2} \frac{\partial \delta}{\partial x} \mathrm{d} (\frac{y}{\hat{\delta}})  
- \nu \hat{u}_\infty \hat{g}^\prime \frac{1}{\hat{\delta}} \bigg|_0^y  &= 0 \\
 \frac{\partial \hat{\delta}}{\partial x} \int_0^1 g  \hat{g}^\prime \hat{\eta} \mathrm{d} \hat{\eta}
- \frac{\partial \delta}{\partial x} \frac{\hat{\delta}^2}{\delta^2} \int_0^1 g^\prime  \hat{\eta}  \mathrm{d} \hat{\eta}
- \frac{\nu}{u_\infty} \hat{g}^\prime \frac{1}{\hat{\delta}} \bigg|_0^1= 0.
\end{align}
The equation optically simplifies by rewriting to;
\begin{align}
\hat{A} \frac{\partial \hat{\delta} }{\partial x} \hat{\delta} - \hat{B} \frac{\partial \delta}{\partial x} \frac{\hat{\delta}^3}{\delta^2}  =  \frac{\nu}{u_\infty} \hat{C}  \label{equ:adjoint_similarity_ode}
\end{align}
by introducing:
\begin{align}
\hat{A}  &= \int_0^1 g  \hat{g}^\prime \frac{y}{\hat{\delta}} \mathrm{d} (\frac{y}{\hat{\delta}}) = \int_0^1 g  \hat{g}^\prime \hat{\eta} \ \mathrm{d} \hat{\eta} \\
\hat{B}  &= \int_0^1 g^\prime \frac{y}{\delta}  \mathrm{d} (\frac{y}{\delta}) = \int_0^1 g^\prime \eta \  \mathrm{d} \eta  = B   \\
\hat{C} &= \hat{g}^\prime(1) - \hat{g}^\prime(0).
\end{align}
Equ. \ref{equ:adjoint_similarity_ode} can be rewritten to;
\begin{align}
C_\mathrm{1} \hat{\delta} \frac{\partial \hat{\delta}}{\partial x} - C_\mathrm{2} \left(  \frac{\hat{\delta}}{\sqrt{a+bx}}\right)^3  = C_\mathrm{3}.
\end{align}
where $C_\mathrm{1} = \hat{A}$, $C_\mathrm{2} = 1/\sqrt{32} \hat{B} \sqrt{(B-2 A)b^3/2 C} \sqrt{u_\infty / \nu}$ and $C_\mathrm{3} = \nu / u_\infty \hat{C}$ are defined. 
%
The equation can be solved to:
\begin{align}
\hat{\delta} &= \sqrt{a+bx} \ R(C_\mathrm{1}, C_\mathrm{2}, C_\mathrm{3}),
\end{align}
where $R$ represents the roots of the characteristic polynomial $R = 2 C_\mathrm{2} z^3 - C_\mathrm{1}  z^2 + 2 C_\mathrm{3}$ and $L$ corresponds to the plate length. The only real root corresponds to:
\begin{align}
R_1 &= \frac{1}{3} \frac{1}{2 C_\mathrm{2}}  \frac{1}{t} \frac{1}{\sqrt[3]{2}}\left[ t^2 + C_\mathrm{1} \sqrt[3]{2} t + 2^{2/3} C_\mathrm{1}^2 \right] 
\hspace{5mm} \mathrm{with} \hspace{5mm} 
t = \sqrt[3]{ 8 C_\mathrm{2}^2 C_\mathrm{3} + 3 \sqrt{3} \hat{t} + 2 C_\mathrm{1}^3} 
\hspace{5mm} \mathrm{and} \hspace{5mm} 
\hat{t} = \sqrt{864 C_\mathrm{2}^4 C_\mathrm{3}^2 + 32 C_\mathrm{2}^2 C_\mathrm{1}^3 C_\mathrm{3}} \\
&= \frac{\sqrt{8}}{3 \sqrt[3]{2}} \frac{b}{ \hat{B} t} \sqrt{\frac{2C}{b \left[B-2 A\right]}} \sqrt{ \frac{\nu}{u_\infty}}  \left[ t^2 + \hat{A} \sqrt[3]{2} t + 2^{2/3} \hat{A} ^2 \right] 
\hspace{5mm} \mathrm{with} \hspace{5mm} 
t = \sqrt[3]{ 2 \left( \hat{B} \sqrt{\frac{B-2 A}{2 C}} \sqrt{ \frac{u_\infty}{ \nu}} \right)^2 \left( \frac{\nu \hat{C}}{u_\infty}\right)+ 3 \sqrt{3} \hat{t} + 2 \hat{A} ^3} \\
& \hspace{1cm}
\hspace{5mm} \mathrm{and} \hspace{5mm} 
\hat{t} = \sqrt{54 \left(  \hat{B} \sqrt{\frac{B-2 A}{2 C}} \sqrt{ \frac{u_\infty}{ \nu}} \right)^4 \left( \frac{\nu \hat{C}}{u_\infty}\right)^2 + 8 \hat{A}^3 \left( \hat{B} \sqrt{\frac{B-2 A}{2 C}} \sqrt{ \frac{u_\infty}{ \nu}} \right)^2  \left( \frac{\nu \hat{C}}{u_\infty} \right) }.
\end{align}
Thus we can estimate the adjoint boundary layer thickness via:
\begin{align}
\hat{\delta} &=  \frac{\sqrt{8}}{3 \sqrt[3]{2}} \frac{b}{ \hat{B} t} \underbrace{ \sqrt{\frac{2C}{b \left[B-2 A \right]}} \sqrt{ \frac{\nu (a + bx)}{u_\infty}} }_{\delta} \left[ ... \right]
\hspace{1cm} \Rightarrow \hspace{1cm} 
\hat{\delta} \propto \delta \propto \sqrt{ \frac{\nu (a+bx)}{u_\infty} },
\end{align}
which is a function of the primal boundary layer thickness and the definition of our adjoint similarity variable reads:
\begin{align}
\hat{\eta} &= \frac{y}{\hat{\delta}} \propto y \sqrt{\frac{u_\infty}{\nu (a+bx)}} = \frac{y}{\delta} = \eta.
\end{align}

\subsection{Adjoint Blasius Equation}
So far, it is unsure if this really simplifies the PDE into an ODE. Besides, the velocity components are not accessible so far. Thus, we take a stream function that directly satisfies the adjoint continuity Equ.
\begin{align}
\hat{u} &= \frac{\partial \hat{\psi}}{\partial y} \\
\hat{v} &= -\frac{\partial \hat{\psi}}{\partial x}.
\end{align}
The potential can be integrated from the first equation, viz.
\begin{align}
\hat{\psi} &= \int_0^y \hat{u} \mathrm{d} y \\
&= \int_0^y \hat{u}_\infty \hat{g} \mathrm{d} y  \\
&= \int_0^{\hat{\eta}} \hat{u}_\infty \hat{g}  \frac{\mathrm{d} y}{\mathrm{d} \hat{\eta}} \mathrm{d} \hat{\eta} \\
&= \sqrt{\frac{\nu \left[a + bx \right] \hat{u}_\infty^2}{u_\infty}} \underbrace{\int_0^{\hat{\eta}} \hat{g}  \mathrm{d} \hat{\eta}}_{\hat{f}(\hat{\eta})},
\end{align}
where we scramble the integral of $\hat{g}$ over $\hat{\eta}$ into the general function $\hat{f}(\hat{\eta})$. Thus, we have a potential that depends on $x$ and $\hat{\eta}$ only and we can compute the necessary derivatives:
\begin{align}
\hat{u} &= \frac{\partial \hat{\psi}}{\partial y} =\sqrt{\frac{\nu \left[a + bx \right] \hat{u}_\infty^2}{u_\infty}} \hat{f}^\prime \frac{\partial \hat{\eta}}{\partial y} = \hat{u}_\infty \hat{f}^\prime \\
\frac{\partial \hat{u} }{\partial x} &= - \frac{1}{2} \hat{u}_\infty \hat{f}^{\prime \prime} y \sqrt{\frac{u_\infty}{\nu \left[ a + bx \right]}} \frac{b}{a + bx} = - \frac{1}{2} \frac{ \hat{u}_\infty b}{a + bx} \hat{f}^{\prime \prime} \hat{\eta} \\
\frac{\partial \hat{u} }{\partial y} &= \hat{u}_\infty \hat{f}^{\prime \prime} \sqrt{\frac{u_\infty}{\nu \left[ a + bx \right]}} \\
\frac{\partial^2 \hat{u} }{\partial y^2} &= \hat{u}_\infty \hat{f}^{\prime \prime \prime} \frac{u_\infty}{\nu \left[ a + bx \right]}.
\end{align}
Inserting them into the adjoint boundary layer equation results in:
\begin{align}
 \frac{1}{2} u_\infty f^\prime \frac{ \hat{u}_\infty b}{a + bx} \hat{f}^{\prime \prime} \hat{\eta}
-  \frac{1}{2} \sqrt{\frac{\nu b^2 u_\infty}{a + bx}} \left[ f^\prime \eta - f \right] \hat{u}_\infty \hat{f}^{\prime \prime} \sqrt{\frac{u_\infty}{\nu \left[ a + bx \right]}}
- \nu \hat{u}_\infty \hat{f}^{\prime \prime \prime} \frac{u_\infty}{\nu \left[ a + bx \right]}
&= \hat{u}_\infty \hat{f}^\prime \frac{1}{2} \frac{ u_\infty b}{a + bx} f^{\prime \prime} \eta \\
%
 \frac{1}{2} u_\infty f^\prime \frac{ \hat{u}_\infty b}{a + bx} \hat{f}^{\prime \prime} \hat{\eta}
-  \frac{1}{2} \frac{ b u_\infty}{a + bx} \left[ f^\prime \eta - f \right] \hat{u}_\infty \hat{f}^{\prime \prime}  
- \hat{u}_\infty \hat{f}^{\prime \prime \prime} \frac{u_\infty}{ \left[ a + bx \right]}
&= \hat{u}_\infty \hat{f}^\prime \frac{1}{2} \frac{ u_\infty b}{a + bx} f^{\prime \prime} \eta \\
%
\frac{1}{2}   f^\prime \frac{ \hat{u}_\infty b}{a + bx} \hat{f}^{\prime \prime} \hat{\eta}
-  \frac{1}{2} \frac{ b  }{a + bx} \left[ f^\prime \eta - f \right] \hat{u}_\infty \hat{f}^{\prime \prime}  
- \hat{u}_\infty \hat{f}^{\prime \prime \prime} \frac{1}{ \left[ a + bx \right]}
&= \hat{u}_\infty \hat{f}^\prime \frac{1}{2} \frac{  b}{a + bx} f^{\prime \prime} \eta \\
%
 \frac{1}{2}   f^\prime \frac{ b}{a + bx} \hat{f}^{\prime \prime} \hat{\eta}
-  \frac{1}{2} \frac{ b  }{a + bx} \left[ f^\prime \eta - f \right] \hat{f}^{\prime \prime}  
- \hat{f}^{\prime \prime \prime} \frac{1}{ \left[ a + bx \right]}
&= \hat{f}^\prime \frac{1}{2} \frac{  b}{a + bx} f^{\prime \prime} \eta \\
%
 \frac{1}{2}   f^\prime  b  \hat{f}^{\prime \prime}  \hat{\eta}
-  \frac{1}{2}  b \left[ f^\prime \eta - f \right] \hat{f}^{\prime \prime}  
- \hat{f}^{\prime \prime \prime} 
&= \hat{f}^\prime \frac{1}{2} b f^{\prime \prime} \eta \\
 f^\prime  b  \hat{f}^{\prime \prime}  \hat{\eta}
- b \left[ f^\prime \eta - f \right] \hat{f}^{\prime \prime}  
- 2 \hat{f}^{\prime \prime \prime} 
&= \hat{f}^\prime b f^{\prime \prime} \eta \\
f^\prime b  \hat{f}^{\prime \prime} \left[ \hat{\eta} - \eta \right]
+ b f  \hat{f}^{\prime \prime}  
- 2 \hat{f}^{\prime \prime \prime} 
&= \hat{f}^\prime b f^{\prime \prime} \eta \\
 b \left[ \hat{\eta} - \eta \right] f^\prime  \hat{f}^{\prime \prime}
+ b f  \hat{f}^{\prime \prime}  
- 2 \hat{f}^{\prime \prime \prime} 
&= b \eta f^{\prime \prime} \hat{f}^\prime
\end{align}
where the right hand side correspond to the additional advection term (RinR) within the adjoint momentum balance.

\subsection{Adjoint Blasius Equation (Alternative Derivation)}
Alternatively, we can (again) directly insert the simplified equation into a Lagrangian. However, the adjoint momentum equations are derived via a variation into the plate normal and tangential velocity. Thus, the following definition of the Lagrangian is intuitive, viz:
\begin{align}
L = \int_{\eta} \hat{f} \left[ - f f^{\prime \prime} - 2 f^{\prime \prime \prime} \right] \mathrm{d} \eta,
\end{align}
but physically non-sense, since the Lagrangian multiplier needs to account for the adjoint velocity which in turn scales with $\hat{f}^\prime$. Knowing the relation between primal plate tangential and normal velocity ($u = f^\prime$, $v =f^\prime \eta - f = u \eta - f$) allows a transformation into the velocity space and supports the interpretation. Thus, an appropriate Lagrangian reeds:
\begin{align}
L = \int_{\eta} \underbrace{\hat{u}}_{\hat{f}^\prime} \left[ - \underbrace{\left( u \eta - v \right)}_{f} \underbrace{ u^{\prime}}_{f^{\prime \prime}} - 2 \underbrace{ u^{\prime \prime}}_{f^{\prime \prime \prime}} \right] \mathrm{d} \eta,
\end{align}
that can now varied in $u$ and $v$.
\begin{align}
\delta_\mathrm{u} L \cdot \delta u + \delta_\mathrm{v} L \cdot \delta v 
&= \int_{\eta} \hat{u} \left[ \left( \delta v - \delta u \eta \right) u^{\prime} + \left(  v -  u \eta \right) \left( \delta u \right)^{\prime} - 2 \left( \delta u \right)^{\prime \prime} \right] \mathrm{d} \eta \\
&= \int_{\eta} \hat{u} \left[ \delta v  u^{\prime} - \delta u \eta  u^{\prime} + v \left( \delta u \right)^{\prime} - u \eta \left( \delta u \right)^{\prime}  - 2 \left( \delta u \right)^{\prime \prime} \right] \mathrm{d} \eta \\
&= \int_{\eta} \delta v  \left[ \hat{u} u^{\prime} \right] + \delta u \left[ - \hat{u} \eta  u^{\prime} -  \left( \hat{u} v \right)^{\prime} + \left( \hat{u} u \eta \right)^{\prime}  - 2 \hat{u}^{\prime \prime} \right] \mathrm{d} \eta \\
&= \int_{\eta} \delta v  \left[ \hat{u} u^{\prime} \right] + \delta u \left[ - \hat{u} \eta  u^{\prime} -  \hat{u}^{\prime} v - \hat{u} v^\prime + \hat{u}^{\prime} u \eta + \hat{u} u^\prime \eta + \hat{u} u  - 2 \hat{u}^{\prime \prime} \right] \mathrm{d} \eta \\
&= \int_{\eta} \delta v  \left[ \hat{u} u^{\prime} \right] + \delta u \left[  -  \hat{u}^{\prime} v - \hat{u} v^\prime + \hat{u}^{\prime} u \eta + \hat{u} u  - 2 \hat{u}^{\prime \prime} \right] \mathrm{d} \eta \\
&= \int_{\eta} \delta v  \left[ \hat{u} u^{\prime} \right] + \delta u \left[  -  \hat{u}^{\prime} \left( u \eta -f  \right) - \hat{u} \left( u \eta -f  \right)^\prime + \hat{u}^{\prime} u \eta + \hat{u} u  - 2 \hat{u}^{\prime \prime} \right] \mathrm{d} \eta \\
&= \int_{\eta} \delta v  \left[ \hat{u} u^{\prime} \right] + \delta u \left[  -  \hat{u}^{\prime} u \eta + \hat{u}^\prime f  - \hat{u} \left( u^\prime \eta + u \eta ^\prime - f^\prime  \right) + \hat{u}^{\prime} u \eta + \hat{u} u  - 2 \hat{u}^{\prime \prime} \right] \mathrm{d} \eta \\
&= \int_{\eta} \delta v  \left[ \hat{u} u^{\prime} \right] + \delta u \left[  -  \hat{u}^{\prime} u \eta + \hat{u}^\prime f  - \hat{u} u^\prime \eta - \hat{u}  u  + \hat{u}  f^\prime + \hat{u}^{\prime} u \eta + \hat{u} u  - 2 \hat{u}^{\prime \prime} \right] \mathrm{d} \eta \\
&= \int_{\eta} \delta v  \left[ \hat{u} u^{\prime} \right] + \delta u \left[ \hat{u}^\prime f  - \hat{u} u^\prime \eta   + \hat{u}  f^\prime  - 2 \hat{u}^{\prime \prime} \right] \mathrm{d} \eta \\
&= \int_{\eta} \delta v  \left[ \hat{f}^\prime f^{\prime \prime} \right] + \delta u \left[ \hat{f}^{\prime \prime} f  - \hat{f}^\prime f^{ \prime \prime} \eta   + \hat{f}^\prime  f^\prime  - 2 \hat{f}^{\prime \prime \prime} \right] \mathrm{d} \eta.
\end{align}
Wo kommt dieser Extra Term her?! Der darf nicht auftauchen. Ergbit auch in den shooting ergebnissen keinen sinn.

%Alternatively, we start with
%\begin{align}
%\delta_{\mathrm{f}^\prime} L \cdot \delta f^\prime
%&= \int_{\eta} \hat{f}^\prime \left[ -\left( \delta f \right) f^{\prime \prime} - f \left( \delta f \right)^{\prime \prime} - 2 \left( \delta f \right)^{\prime \prime \prime} \right] \mathrm{d} \eta \\
%&= \int_{\eta} \left( \delta f \right) \left[ \hat{f}^\prime f^{\prime \prime} \right]+ \left( \delta f \right)^\prime  \left[ \left( \hat{f}^\prime f \right)^{\prime} - 2 \hat{f}^{\prime \prime \prime} \right] \mathrm{d} \eta \\
%&= \int_{\eta} \left( \delta f \right) \left[ \hat{f}^\prime f^{\prime \prime} \right]+ \left( \delta f \right)^\prime  \left[ \hat{f}^{\prime \prime} f + \hat{f}^\prime f^\prime - 2 \hat{f}^{\prime \prime \prime} \right] \mathrm{d} %\eta.
%\end{align}
%Choosing $\delta f = (\eta + f^\prime / f^{\prime \prime}) \delta f^\prime$ one ends up with
%\begin{align}
%\delta_{\mathrm{f}^\prime} L \cdot \delta f^\prime
%&= \int_{\eta}  \left( \delta f \right)^\prime  \left[ \hat{f}^{\prime \prime} f - \hat{f}^\prime f^{\prime \prime} %\eta - 2 \hat{f}^{\prime \prime \prime} \right] \mathrm{d} \eta,
%\end{align}
%that equals the adjoint Blasius Equ. The relation between $\delta f$ and $\delta f^\prime$ results from the definition %of $v$, viz.
%\begin{align}
%v = f^\prime \eta - f &= u \eta - f \\
%\Leftrightarrow \delta v &= \delta f^\prime \eta - \delta f \\
%\frac{\delta f }{\delta f^\prime} &= \eta - \frac{\delta v}{\delta f^\prime} = \eta - \frac{\delta v}{\delta u}
%\end{align}
%Assuming that $u \approx f^\prime$ and $v \approx -f$, a Taylor series expansion read $\delta u \approx \partial u / %\partial \eta \delta \eta$ as well as $\delta v \approx \partial v / \partial \eta \delta \eta$, that results in:
%\begin{align}
%\frac{\delta v}{\delta u} = \frac{-f^\prime \delta \eta}{f^{\prime \prime}\delta \eta} = - \frac{f^\prime}{f^{\prime %\prime}}.
%\end{align}.

The next derivation starts with with
\begin{align}
\delta_{\mathrm{f}^\prime} L \cdot \delta f^\prime
&= \int_{\eta} \hat{f}^\prime \left[ - f \left( \delta f^\prime \right)^\prime - 2 \left( \delta f^\prime \right)^{\prime \prime} \right] \mathrm{d} \eta \\
&= \int_{\eta} \delta f^\prime \left[ \left( f \hat{f}^\prime \right)^\prime - 2 \hat{f}^{\prime \prime \prime} \right] \mathrm{d} \eta.
\end{align}
Mind that we know $f = f^\prime \eta - v$ and thus the derivative can be rewritten to:
\begin{align}
\delta_{\mathrm{f}^\prime} L \cdot \delta f^\prime
&= \int_{\eta} \delta f^\prime \left[ \left( \left( f^\prime \eta - v \right) \hat{f}^\prime \right)^\prime - 2 \hat{f}^{\prime \prime \prime} \right] \mathrm{d} \eta \\
&= \int_{\eta} \delta f^\prime \left[ \left( f^\prime \eta - v \right)^\prime \hat{f}^\prime + \left( f^\prime \eta - v \right) \hat{f}^{\prime \prime}  - 2 \hat{f}^{\prime \prime \prime} \right] \mathrm{d} \eta \\
&= \int_{\eta} \delta f^\prime \left[ \left( f^{\prime  \prime} \eta + f^\prime - \frac{\mathrm{d} v}{\mathrm{d} \eta}  \right)  \hat{f}^\prime + f \hat{f}^{\prime \prime}  - 2 \hat{f}^{\prime \prime \prime} \right] \mathrm{d} \eta \\
&= \int_{\eta} \delta f^\prime \left[ \left( f^{\prime  \prime} \eta + f^\prime - f^\prime \right)  \hat{f}^\prime + f \hat{f}^{\prime \prime}  - 2 \hat{f}^{\prime \prime \prime} \right] \mathrm{d} \eta \\
&= \int_{\eta} \delta f^\prime \left[ f^{\prime  \prime} \eta  \hat{f}^\prime + f \hat{f}^{\prime \prime}  - 2 \hat{f}^{\prime \prime \prime} \right] \mathrm{d} \eta
\end{align}

The final approach starts with the Lagrangian in Euclidean space, viz.
\begin{align}
L &= ...
+ \int_\mathrm{x_\mathrm{1}} \int_\mathrm{x_\mathrm{2}} \hat{v}_\mathrm{1} R_\mathrm{1}^\mathrm{BL} + \hat{v}_\mathrm{2} R_\mathrm{2}^\mathrm{BL} \mathrm{d} x_\mathrm{2} \mathrm{d} x_\mathrm{1} \\
&= ... + \int_\mathrm{x_\mathrm{2}} \int_\mathrm{\eta} \left[ \hat{v}_\mathrm{1} R_\mathrm{1}^\mathrm{BL} + \hat{v}_\mathrm{2} R_\mathrm{2}^\mathrm{BL} \right] \sqrt{\frac{\nu (a + b x_\mathrm{1})}{V_\mathrm{1}}} \mathrm{d} \eta \mathrm{d} x_\mathrm{1} \\
&= ... + \int_\mathrm{x_\mathrm{2}} \int_\mathrm{\eta} \hat{f}^\prime \hat{V}_\mathrm{1} \left[ -2 f^{\prime \prime \prime} - f f^{\prime \prime}\right] \frac{V_\mathrm{1}^2}{\nu (a + b x_\mathrm{1})} \sqrt{\frac{\nu (a + b x_\mathrm{1})}{V_\mathrm{1}}} \mathrm{d} \eta \mathrm{d} x_\mathrm{1} \\
&= ... + \int_\mathrm{x_\mathrm{2}} \int_\mathrm{\eta} \hat{f}^\prime \left[ -2 f^{\prime \prime \prime} - f f^{\prime \prime}\right] \sqrt{\frac{V_\mathrm{1}^3 \hat{V}_\mathrm{1}^2}{\nu (a + b x_\mathrm{1})}} \mathrm{d} \eta \mathrm{d} x_\mathrm{1} \\
&= ... + \int_\mathrm{x_\mathrm{2}} \int_\mathrm{\eta} \hat{f}^\prime \left[ -2 f^{\prime \prime \prime} - f^\prime f^{\prime \prime} \eta + (f^\prime \eta - f ) f^{\prime \prime}\right]  \mathrm{d} \eta \sqrt{\frac{V_\mathrm{1}^3 \hat{V}_\mathrm{1}^2}{\nu (a + b x_\mathrm{1})}} \mathrm{d} x_\mathrm{1}
\end{align}
The total variation of this expression reads:
\begin{align}
\delta L &= ... + \int_\mathrm{x_\mathrm{2}} \int_\mathrm{\eta} \hat{f}^\prime \delta \left[ -2 f^{\prime \prime \prime} - f^\prime f^{\prime \prime} \eta + (f^\prime \eta - f ) f^{\prime \prime}\right]  \mathrm{d} \eta \sqrt{\frac{V_\mathrm{1}^3 \hat{V}_\mathrm{1}^2}{\nu (a + b x_\mathrm{1})}} \mathrm{d} x_\mathrm{1} \\
\delta L &= ... + \int_\mathrm{x_\mathrm{2}} \int_\mathrm{\eta} \hat{f}^\prime \left[ -2 (\delta f)^{\prime \prime \prime} - \delta \left[ f^\prime f^{\prime \prime} \eta\right] +  \delta \left[ (f^\prime \eta - f ) f^{\prime \prime} \right] \right]  \mathrm{d} \eta \sqrt{\frac{V_\mathrm{1}^3 \hat{V}_\mathrm{1}^2}{\nu (a + b x_\mathrm{1})}} \mathrm{d} x_\mathrm{1}
\end{align}


\subsection{Continuous Investigation of Adjoint Blasius Equation}
\paragraph{Without Advection}
A strong similarity between the adjoint Blasius Equ. and a thermal boundary layer arises, when the advection term on the r.h.s. of the adjoint Blasius Equ. is negleted. However, a switch in sign of is observed due to the  inverse convection characteristics. In combination with $f = -2 f^{\prime \prime \prime} / f^{\prime \prime}$ we find.
\begin{align}
-2 \hat{f}^{\prime \prime \prime} - 2 \frac{ f^{\prime \prime \prime}}{f^{\prime \prime}} \hat{f}^{\prime \prime } &= 0 \\
\Rightarrow \frac{\hat{f}^{\prime \prime \prime}}{\hat{f}^{\prime \prime}} &= - \frac{ f^{\prime \prime \prime}}{f^{\prime \prime}}.
\end{align}
This ODE can be solved w.r.t. $\hat{f}^\prime$, viz.
\begin{align}
\frac{\mathrm{d} \hat{f}^{\prime \prime}}{\mathrm{d} \eta} \frac{1}{\hat{f}^{\prime \prime}} &= -\frac{\mathrm{d} f^{\prime \prime}}{\mathrm{d} \eta} \frac{1}{f^{\prime \prime}} \\
\mathrm{ln}\left(  \hat{f}^{\prime \prime} \right) &= -\mathrm{ln}\left(  f^{\prime \prime} \right) C_\mathrm{1} \\
\hat{f}^{\prime \prime} &= \frac{1}{f^{\prime \prime}} C_\mathrm{1}.
\end{align}
The equation can further integrated to obtain the final solution:
\begin{align}
\hat{f}^{\prime} &= \int_0{\eta} \frac{1}{f^{\prime \prime}} C_\mathrm{1} \mathrm{d} \eta + C_\mathrm{2}.
\end{align}
The constants result from the boundary conditions:
\begin{align}
\hat{f}^\prime (\eta = 0) = 0 \Rightarrow C_\mathrm{2} &= 0 \\
\hat{f}^\prime (\eta = \infty) = 1 \Rightarrow C_\mathrm{1}  &= \frac{1}{\int_0^{\infty} \frac{1}{f^{\prime \prime}} \mathrm{d} \eta}.
\end{align}
Obviously the problem is ill-posed, since the term $1 / f^{\prime \prime} \longrightarrow \infty$ for $\eta \longrightarrow \infty$. This problem is caused by the negative sign on the r.h.s. which in turn originates from the backward flow characteristics of adjoint Navier-Stokes.

%\subsection{Adjoint Blasius Equation}
%The definition of $\hat{u} = \partial \hat{\psi}^* / \partial y$ and $\hat{v} = - \partial \hat{\psi}^* / \partial x$ by knowing $\hat{\psi} := \hat{\psi}(x, y, \hat{\eta}^*) = \beta \, \sqrt{1-x} \, \, \hat{f}^* (\hat{\eta}^*)$ and $\hat{\eta}^* := \hat{\eta}^* (x, y) = \alpha \, y / \sqrt{1-x}$ yields:
%\begin{itemize}
%\item $\hat{u} \rightarrow \hat{a} \hat{b} \hat{f}^\prime$
%\item $\partial \hat{u} / \partial x \rightarrow \hat{a} \hat{b} \hat{f}^{\prime \prime} \hat{b} y \frac{1}{2} (1-x)^{-3/2}$
%\item $\partial \hat{u} / \partial y \rightarrow \hat{a} \hat{b} \hat{f}^{\prime \prime} \hat{b} (1-x)^{-1/2}$
%\item $\partial \hat{u}^2 / \partial y^2 \rightarrow \hat{a} \hat{b} \hat{f}^{\prime \prime \prime} \hat{b} (1-x)^{-1/2} \hat{b} (1-x)^{-1/2}$
%%\item $v \rightarrow - a \frac{1}{2} x^{-1/2} f - a x^{1/2} f^\prime y b \left(-\frac{1}{2}\right) x^{-3/2}$
%\end{itemize}
%for each term in the boundary layer equation. In the absence of pressure gradient this results in:
%\begin{align}
%-u \frac{\partial \hat{u}}{\partial x} 
%-v \frac{\partial \hat{u}}{\partial y}
%+\hat{u} \frac{\partial u}{\partial x} 
%- \nu \frac{\partial^2 \hat{u}}{\partial y^2} 
%&= 0 \\
%- a b f^\prime \hat{a} \hat{b} \hat{f}^{\prime \prime} \hat{b} y \frac{1}{2} (1-x)^{-3/2}
%+ a \frac{1}{2} x^{-1/2} f + a x^{1/2} f^\prime y b \left(-\frac{1}{2}\right) x^{-3/2} \hat{a} \hat{b} \hat{f}^{\prime \prime} \hat{b} (1-x)^{-1/2} & \\
%- \hat{a} \hat{b} \hat{f}^\prime a b f^{\prime \prime} b y \frac{1}{2} x^{-3/2}
%- \hat{a} \hat{b} \hat{f}^{\prime \prime \prime} \hat{b} (1-x)^{-1/2} \hat{b} (1-x)^{-1/2}
%&= 0 \\
%- \frac{1}{2} a b \hat{a} \hat{b}^2 f^\prime \hat{f}^{\prime \prime} y (1-x)^{-3/2}
%+ \left[ x^{-1/2} f - x^{1/2} f^\prime y b x^{-3/2} \right]  \frac{1}{2} a \hat{a} \hat{b} \hat{f}^{\prime \prime} \hat{b} (1-x)^{-1/2} & \\
%- \frac{1}{2} a b^2 \hat{a} \hat{b} \hat{f}^\prime f^{\prime \prime} y x^{-3/2}
%- \hat{a} \hat{b}^3 \hat{f}^{\prime \prime \prime} (1-x)^{-1}
%&= 0 \\
%- \frac{1}{2} a b \hat{a} \hat{b}^2 f^\prime \hat{f}^{\prime \prime} y (1-x)^{-3/2}
%+ \frac{1}{2} a \hat{a} \hat{b}^2 x^{-1/2} f \hat{f}^{\prime \prime} (1-x)^{-1/2} 
%- \frac{1}{2} a b \hat{a} \hat{b}^2  f^\prime y  x^{-1} \hat{f}^{\prime \prime} (1-x)^{-1/2} & \\
%- \frac{1}{2} a b^2 \hat{a} \hat{b} \hat{f}^\prime f^{\prime \prime} y x^{-3/2}
%- \hat{a} \hat{b}^3 \hat{f}^{\prime \prime \prime} (1-x)^{-1}
%&= 0 \\
%- \frac{1}{2} a b \hat{a} \hat{b}^2 f^\prime \hat{f}^{\prime \prime} y^3 (1-x)^{-3/2}
%+ \frac{1}{2} a \hat{a} \hat{b}^2 x^{-1/2} f \hat{f}^{\prime \prime} y^2 (1-x)^{-1/2} 
%- \frac{1}{2} a b \hat{a} \hat{b}^2  f^\prime y^3  x^{-1} \hat{f}^{\prime \prime} (1-x)^{-1/2} & \\
%- \frac{1}{2} a b^2 \hat{a} \hat{b} \hat{f}^\prime f^{\prime \prime} y^3 x^{-3/2}
%- \hat{a} \hat{b}^3 \hat{f}^{\prime \prime \prime} y^2 (1-x)^{-1}
%&= 0 \\
%- \frac{1}{2} a b \hat{a} \hat{b}^2 f^\prime \hat{f}^{\prime \prime} \hat{\eta}^3 / \hat{b}^3
%+ \frac{1}{2} a \hat{a} \hat{b}^2 f \hat{f}^{\prime \prime} \eta / b \hat{\eta} / \hat{b}
%- \frac{1}{2} a b \hat{a} \hat{b}^2  f^\prime \eta^2 / b^2 \hat{f}^{\prime \prime} \hat{\eta} / \hat{b} & \\
%- \frac{1}{2} a b^2 \hat{a} \hat{b} \hat{f}^\prime f^{\prime \prime} \eta^3 / b^3
%- \hat{a} \hat{b}^3 \hat{f}^{\prime \prime \prime} \hat{\eta}^2 / \hat{b}^2
%&= 0 \\
%- \frac{1}{2} a \hat{a} \frac{b}{\hat{b}} f^\prime \hat{f}^{\prime \prime} \hat{\eta}^3 
%+ \frac{1}{2} a \hat{a} \frac{\hat{b}}{b} f \hat{f}^{\prime \prime} \eta \hat{\eta} 
%- \frac{1}{2} a \hat{a} \frac{\hat{b}}{b}  f^\prime \eta^2 \hat{f}^{\prime \prime} \hat{\eta}  & \\
%- \frac{1}{2} a \hat{a} \frac{\hat{b}}{b} \hat{f}^\prime f^{\prime \prime} \eta^3 
%- \hat{a} \hat{b} \hat{f}^{\prime \prime \prime} \hat{\eta}^2
%&= 0 \\
%- \frac{b^2}{\hat{b}^2} f^\prime \hat{f}^{\prime \prime} \hat{\eta}^3 
%+ f \hat{f}^{\prime \prime} \eta \hat{\eta} 
%- f^\prime \eta^2 \hat{f}^{\prime \prime} \hat{\eta} 
%- \hat{f}^\prime f^{\prime \prime} \eta^3 
%- 2 \frac{b}{a} \hat{f}^{\prime \prime \prime} \hat{\eta}^2
%&= 0
%\end{align}


%The well known first order Blasius equation is derived from a similarity transformation of the cartesian coordinates $x_\mathrm{i}$  into a dimensionless wall (normal) distance $\eta^* := \eta^* (x_\mathrm{1}, x_\mathrm{2}, \beta) = \beta \, x_\mathrm{2} / \sqrt{x_\mathrm{1}}$.
%%
%Subsequently, a stream function is defined $\psi := \psi(x_\mathrm{1}, x_\mathrm{2}, \eta^*, \alpha, \beta) = \alpha \, \sqrt{x_\mathrm{1}} \, \, f^* (\eta^*)$ as a function of a dimensionless function $f^*$ which in turn depends on the dimensionless wall distance.
%%
%The depence of $\psi^*$ and $\eta^*$ on $x_\mathrm{1}$ are anticipated from experience and the variables $\alpha$ and $\beta$ serve as a closure of dimensionality, viz. $v_\mathrm{1} = \partial \psi / \partial x_\mathrm{2}$ and $v_\mathrm{2} = - \partial \psi / \partial x_\mathrm{1}$.
%%
%This relationship fullfills Equ. \ref{equ:primal_bounday_layer_mass1_first}. In the absence of pressure gradients, the primal $x_\mathrm{1}$ boundary layer Equ. \ref{equ:primal_bounday_layer_mome1_first} simplifies to:
%\begin{align}
%v_\mathrm{1} \frac{\partial v_\mathrm{1}}{\partial x_\mathrm{1}} 
%+ v_\mathrm{2} \frac{\partial v_\mathrm{1}}{\partial x_\mathrm{2}}
%- \nu \frac{\partial^2 v_\mathrm{1}}{\partial x_\mathrm{2}^2} 
%&= 0 \\
%\Leftrightarrow \hspace{5mm}
%- 2 \nu \frac{\beta}{\alpha} f^{\prime \prime \prime}
%- f f^{\prime \prime}
%&= 0 \label{equ:primal_blasius}
%\end{align}
%and offers choices for $\alpha$ and $\beta$, since $\nu \, \beta \, / \alpha =  \pm 1$. We choose $\alpha = \sqrt{ V_\mathrm{1} \, \nu}$ and $\beta = \sqrt{V_\mathrm{1} / \nu}$ in accordance with the $V_\mathrm{1}$ bulk or reference value from Tab. \ref{tab:reference_values}.
%
%An adjoint to Equ. \ref{equ:primal_blasius} is obtained following the same recipe that differs in the dependence of the lateral plate coordinate $x_\mathrm{1}$ only.
%%
%This is motivated by the inverted convective physics within the adjoint Equ. \ref{equ:adjoint_momentum}.
%%
%Thus, we define an adjoint dimensionless wall spacing $\hat{\eta}^* := \hat{\eta}^* (x_\mathrm{1}, x_\mathrm{2}, \hat{\beta}) = \hat{\beta} \, x_\mathrm{2} / \sqrt{1 - x_\mathrm{1}}$ and stream function $\hat{\psi} := \hat{\psi} (x_\mathrm{1}, x_\mathrm{2}, \hat{\eta}^*, \hat{\alpha}, \hat{\beta}) = \hat{\alpha} \, \sqrt{1-x_\mathrm{1}} \, \, \hat{f}^* (\hat{\eta}^*)$.
%%
%Again, the variables $\hat{\alpha}$ and $\hat{\beta}$ serve as a closure of dimensionality, viz. $\hat{v}_\mathrm{1} = \partial \hat{\psi} / \partial x_\mathrm{2}$ and $\hat{v}_\mathrm{2} = - \partial \hat{\psi} / \partial x_\mathrm{1}$.
%%
%Mind that the primal and adjoint dimensionless wall distance is related, viz. $\hat{\eta} = (\hat{\beta} / \beta) \, t(x_\mathrm{1}) \, \eta$ where $t(x_\mathrm{1}) = \sqrt{x_\mathrm{1} / (1-x_\mathrm{1})}$ scrambles a transformation function.
%%
%In the absence of adjoint pressure gradients, the adjoint $x_\mathrm{1}$ boundary layer Equ. \ref{equ:adjoint_bounday_layer_mome1_first} simplifies to:
%\begin{align}
%- v_\mathrm{1} \frac{\partial \hat{v}_\mathrm{1}}{\partial x_\mathrm{1}} 
%- v_\mathrm{2} \frac{\partial \hat{v}_\mathrm{1}}{\partial x_\mathrm{2}}
%+ \hat{v}_\mathrm{1} \frac{\partial v_\mathrm{1}}{\partial x_\mathrm{1}} 
%- \nu \frac{\partial^2 \hat{v}_\mathrm{1}}{\partial x_\mathrm{2}^2} 
%&= 0 \\
%\Leftrightarrow \hspace{5mm}
%- 2 \frac{\beta}{\alpha} \hat{\eta}^2 \hat{f}^{\prime \prime \prime}
%+ \hat{f}^{\prime \prime} \left[ f \eta \hat{\eta} 
%- f^\prime \left( \frac{\beta^2}{\hat{\beta}^2} \hat{\eta}^3
%+ \eta^2  \hat{\eta} \right) \right]
%- f^{\prime \prime} \eta^3  \hat{f}^\prime
%&= \label{equ:adjoint_blasius_first} 0.
%\end{align}
%Interestingly, Equ. \ref{equ:adjoint_blasius_first} is independent from $\hat{\alpha}$ that adjusts the dimension of the adjoint velocity which in turn depends on the underlying objective.
%%
%The scaling factor for the adjoint boundary layer thickness has to have the same dimension, viz. ($\hat{\beta} = \beta$) and we end up with:
%\begin{align}
%- 2 \hat{\eta}^2 \hat{f}^{\prime \prime \prime}
%+ \hat{f}^{\prime \prime} \left[ f \eta \hat{\eta} 
%- f^\prime \left( \hat{\eta}^3
%+ \eta^2  \hat{\eta} \right) \right]
%- f^{\prime \prime} \eta^3  \hat{f}^\prime
%&= 0.
%\end{align}
%Remembering the relation between $\eta$ and $\hat{\eta}$, viz.
%\begin{align}
%- 2 \hat{f}^{\prime \prime \prime}
%+ \left[f \, t - f^\prime \eta \left( \frac{1}{t} + t \right) \right] \hat{f}^{\prime \prime}
%- f^{\prime \prime} \eta t^2 \hat{f}^\prime
%= 0 \label{equ:adjoint_blasius}.
%\end{align}
%Equ. \ref{equ:adjoint_blasius} can be solved for $\hat{f}(\eta, t)$ under given $f(\eta)$, $\eta$ and $t$.

%\begin{align}
%L = \int \hat{f} \left[-2 \frac{\partial^3 f}{\partial \eta^3} - f \frac{\partial^2 f}{\partial \eta} \right] \mathrm{d} \eta
%\end{align}
%
%\begin{align}
%\delta_\mathrm{\eta} L \cdot \delta \eta &= \int \hat{f} \left[ -2 \frac{\partial^3 (\delta f)}{\partial \eta^3} - \delta f \frac{\partial^2 f}{\partial \eta^2} - f \frac{\partial^2 (\delta f)}{\partial \eta^2} \right] \mathrm{d} \eta \\
%& = \left[ 2 \left( \frac{ \partial \hat{f}}{\partial \eta } \frac{\partial (\delta f)}{\partial \eta} - \hat{f} \frac{\partial^2 (\delta f)}{\partial \eta^2} - \frac{ \partial^2 \hat{f}}{\partial \eta^2} \delta f \right) - \hat{f} f \frac{\partial (\delta f)}{\partial \eta} + \frac{ \partial \hat{f} f}{\partial \eta} (\delta f) \right] \label{equ:blasius_boundary} \\
%& + \int \delta f \left[ 2 \frac{\partial^3 \hat{f}}{\partial \eta^3} - \hat{f} \frac{\partial^2 f}{\partial \eta^2} - \frac{\partial^2 ( \hat{
%f} f)}{\partial \eta^2} \right] \mathrm{d} \eta
%\end{align}
%
%The volume term simplifies to
%\begin{align}
%2 \frac{\partial^3 \hat{f}}{\partial \eta^3} - \hat{f} \frac{\partial^2 f}{\partial \eta} - \frac{\partial^2 \hat{f}}{\partial \eta^2} f - 2 \frac{\partial \hat{f}}{\partial \eta} \frac{\partial f}{\partial \eta}  - \hat{f} \frac{\partial^2 f}{\partial \eta^2} &= 0\\
%%2 \frac{\partial^3 \hat{f}}{\partial \eta^3} - \frac{\partial^2 \hat{f}}{\partial \eta^2} f - 2 \frac{\partial \hat{f}}{\partial \eta} \frac{\partial f}{\partial \eta} - 2 \hat{f} \frac{\partial^2 f}{\partial \eta^2} &= 0 \\
%%a_\mathrm{3} \hat{f}^{(3)} + a_\mathrm{2} \hat{f}^{(2)} + a_\mathrm{1} \hat{f}^{(1)} + a_\mathrm{0} \hat{f}^{(0)} &= 0 \\
%\sum_\mathrm{i=0}^{3} a_\mathrm{i} \hat{f}^{(i)} &= 0,
%\end{align}
%where $a_\mathrm{3} = 2$, $a_\mathrm{2} = -f$, $a_\mathrm{1} = -2 f^{(1)}$ and $a_\mathrm{0} = -2 f^{(2)}$. A variation of the primal BC reveal $\delta f = 0$ and $( \delta f)^\prime = 0$  at $\eta = 0$ as well as $( \delta f)^\prime = 0$ along with $\eta \rightarrow \infty$. Thus, Equ. \ref{equ:blasius_boundary} yields $\hat{f} = 0|_{\eta = 0}$ and $\hat{f} = 0|_{\eta \rightarrow \infty}$ as well as $\hat{f}^{\prime \prime} = \hat{f}^\prime f /2 |_{\eta \rightarrow \infty}$. 
%Since no analytic solution is available for the forward problem ($f$), the backward solution ($\hat{f}$) is also approximated numerically based on a shooting method. 

==> tex/derivations.tex <==
\section{Calculation Area}
\subsection{Primal Simplification}
Primal non-dimensional equations:
\begin{align}
R_\mathrm{1}^*:&  \hspace{3cm}  
v_\mathrm{1}^* \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1} V_\mathrm{1}}{L} 
+ v_\mathrm{2}^* \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{2}^*}\frac{V_\mathrm{2} V_\mathrm{1}}{\delta} 
+ \frac{1}{L}\frac{\partial}{\partial x_\mathrm{1}^*} \left[ \frac{p^*}{\rho} P - \nu \left( \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1}}{L} +  \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1}}{L} \right) \right] \nonumber \\
&\hspace{4cm} 
+ \frac{1}{\delta} \frac{\partial}{\partial x_\mathrm{2}^*} \left[ - \nu \left( \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{1}}{\delta} +  \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{2}}{L} \right) \right] = 0 \\
R_\mathrm{2}^*:&  \hspace{3cm} 
v_\mathrm{1}^* \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1} V_\mathrm{2}}{L} 
+ v_\mathrm{2}^* \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{2} V_\mathrm{2}}{\delta} 
+ \frac{1}{L} \frac{\partial}{\partial x_\mathrm{1}^*} \left[ - \nu \left( \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{2}}{L} +  \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{1}}{\delta} \right) \right] \nonumber \\
&\hspace{4cm} 
+ \frac{1}{\delta} \frac{\partial}{\partial x_\mathrm{2}^*} \left[ \frac{p^*}{\rho} P - \nu \left( \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{2}}{\delta} +  \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{2}}{\delta} \right) \right] = 0 \\
Q^*:& \hspace{4cm} 
-\frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1}}{L}
-\frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{2}}{\delta}
= 0.
\end{align}
Assuming $V_\mathrm{2} \propto V_\mathrm{1} \delta / L$:
\begin{align}
R_\mathrm{1}^*:&  \hspace{3cm}  
v_\mathrm{1}^* \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1} V_\mathrm{1}}{L} 
+ v_\mathrm{2}^* \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{2}^*}\frac{V_\mathrm{1} \delta V_\mathrm{1}}{\delta L} 
+ \frac{1}{L}\frac{\partial}{\partial x_\mathrm{1}^*} \left[ \frac{p^*}{\rho} P - \nu \left( \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1}}{L} +  \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1}}{L} \right) \right] \nonumber \\
&\hspace{4cm} 
+ \frac{1}{\delta} \frac{\partial}{\partial x_\mathrm{2}^*} \left[ - \nu \left( \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{1}}{\delta} +  \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1} \delta}{L L} \right) \right] = 0 \\
R_\mathrm{2}^*:&  \hspace{3cm} 
v_\mathrm{1}^* \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1} V_\mathrm{1} \delta}{L L} 
+ v_\mathrm{2}^* \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{1} \delta V_\mathrm{1} \delta}{\delta L L} 
+ \frac{1}{L} \frac{\partial}{\partial x_\mathrm{1}^*} \left[ - \nu \left( \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1} \delta}{L L} +  \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{1}}{\delta} \right) \right] \nonumber \\
&\hspace{4cm} 
+ \frac{1}{\delta} \frac{\partial}{\partial x_\mathrm{2}^*} \left[ \frac{p^*}{\rho} P - \nu \left( \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{1} \delta}{\delta L} +  \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{1} \delta}{\delta L} \right) \right] = 0 \\
Q^*:& \hspace{4cm} 
-\frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1}}{L}
-\frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{1} \delta}{\delta L}
= 0.
\end{align}
We end up with:
\begin{align}
R_\mathrm{1}^*:&  \hspace{3cm}  
v_\mathrm{1}^* \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*}
+ v_\mathrm{2}^* \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{2}^*}
+ \frac{\partial}{\partial x_\mathrm{1}^*} \left[ p^* \frac{P }{\rho V_\mathrm{1} V_\mathrm{1}} - \frac{\nu}{V_\mathrm{1} L} \left( \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*} +  \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \right) \right] \nonumber \\
&\hspace{4cm} 
+ \frac{\partial}{\partial x_\mathrm{2}^*} \left[- \frac{\nu}{V_\mathrm{1} L} \left( \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{L^2}{\delta^2} +  \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \right) \right] = 0 \\
R_\mathrm{2}^*:&  \hspace{3cm} 
v_\mathrm{1}^* \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{1}^*}
+ v_\mathrm{2}^* \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} 
+ \frac{\partial}{\partial x_\mathrm{1}^*} \left[- \frac{\nu}{V_\mathrm{1} L}  \left( \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{1}^*} +  \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{L^2}{\delta^2} \right) \right] \nonumber \\
&\hspace{4cm} 
+ \frac{\partial}{\partial x_\mathrm{2}^*} \left[ p^* \frac{P }{\rho V_\mathrm{1} V_\mathrm{1}} \frac{L^2}{\delta^2} - \frac{\nu}{V_\mathrm{1} L} \left( \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{L^2}{\delta^2} +  \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{L^2}{\delta^2} \right) \right] = 0 \\
Q^*:& \hspace{4cm} 
-\frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*} 
-\frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} 
= 0.
\end{align}

\subsection{Adjoint Derivation}
General Lagrangian reads:
\begin{align}
L &= \int_\mathrm{\Gamma} j_\mathrm{\Gamma_\mathrm{O}} \mathrm{d} \Gamma \\
& + \int_{\mathrm{\Gamma}_\mathrm{in}} \hat{v_\mathrm{i}} \left[ v_\mathrm{i} - n_\mathrm{i} v_\mathrm{i}^\mathrm{in} \right] \hat{p} \frac{\partial p}{\partial n} \mathrm{d} \Gamma  \\
& + \int_{\mathrm{\Gamma}_\mathrm{out}} \hat{v_\mathrm{i}} \left[ \frac{\partial v_\mathrm{i}}{\partial n} \right] + \hat{p} \frac{\partial p}{\partial n} \mathrm{d} \Gamma \\
& + \int_{\mathrm{\Gamma}_\mathrm{wall}} \hat{v_\mathrm{i}} v_\mathrm{i} + \hat{p} \frac{\partial p}{\partial n} \mathrm{d} \Gamma \\
& + \int_{\Omega} j_\mathrm{\Omega_\mathrm{O}} + \hat{v}_\mathrm{i} \left[ v_\mathrm{k} \frac{\partial v_\mathrm{i}}{\partial x_\mathrm{k}} + \frac{\partial}{\partial x_\mathrm{k}} \left[ \frac{p}{\rho} \delta_\mathrm{ik} - 2 \nu S_\mathrm{ik} \right] \right] - \hat{p} \frac{\partial v_\mathrm{i}}{\partial x_\mathrm{i}}\mathrm{d} \Omega.
\end{align}
Derivative in velocity direction:
\begin{align}
\delta_\mathrm{v_\mathrm{i}} L \cdot \delta v_\mathrm{i} &= \int_\mathrm{\Gamma} \frac{\partial j_\mathrm{\Gamma_\mathrm{O}}}{\partial v_\mathrm{i}} \delta v_\mathrm{i} \mathrm{d} \Gamma \\
& + \int_{\mathrm{\Gamma}_\mathrm{in}} \hat{v_\mathrm{i}} (\delta v_\mathrm{i}) \mathrm{d} \Gamma  \\
& + \int_{\mathrm{\Gamma}_\mathrm{out}} \hat{v_\mathrm{i}} \frac{\partial (\delta v_\mathrm{i})}{\partial n} \mathrm{d} \Gamma \\
& + \int_{\mathrm{\Gamma}_\mathrm{wall}} \hat{v_\mathrm{i}} (\delta v_\mathrm{i}) \mathrm{d} \Gamma \\
& + \int_{\Omega} \frac{\partial j_\mathrm{\Omega_\mathrm{O}}}{\partial v_\mathrm{i}} \delta v_\mathrm{i} + \hat{v}_\mathrm{i} \left[ \delta v_\mathrm{k} \frac{\partial v_\mathrm{i}}{\partial x_\mathrm{k}} + v_\mathrm{k} \frac{\partial (\delta v_\mathrm{i})}{\partial x_\mathrm{k}} - 2 \nu \frac{\partial (\delta S_\mathrm{ik})}{\partial x_\mathrm{k}} \right] - \hat{p} \frac{\partial (\delta v_\mathrm{i})}{\partial x_\mathrm{i}}\mathrm{d} \Omega,
\end{align}
can be rearranged to:
\begin{align}
\delta_\mathrm{v_\mathrm{i}} L \cdot \delta v_\mathrm{i} &= 
\int_{\mathrm{\Gamma}_\mathrm{in}} \hat{v_\mathrm{i}} (\delta v_\mathrm{i}) \mathrm{d} \Gamma  \\
& + \int_{\mathrm{\Gamma}_\mathrm{out}} \hat{v_\mathrm{i}} \frac{\partial (\delta v_\mathrm{i})}{\partial n} \mathrm{d} \Gamma \\
& + \int_{\mathrm{\Gamma}_\mathrm{wall}} \hat{v_\mathrm{i}} (\delta v_\mathrm{i}) \mathrm{d} \Gamma \\
& + \int_{\mathrm{\Gamma}}(\delta v_\mathrm{i}) \left[ \frac{\partial j_\mathrm{\Gamma_\mathrm{O}}}{\partial v_\mathrm{i}} + v_\mathrm{k} \hat{v}_\mathrm{i} n_\mathrm{k} + 2 \nu \hat{S}_\mathrm{ik}n_\mathrm{k} - \hat{p} n_\mathrm{i} \right] - (\delta S_\mathrm{ik}) \hat{v}_\mathrm{i} \nu   \mathrm{d} \Gamma \\
& + \int_{\Omega} \delta v_\mathrm{i} \left[ \frac{\partial j_\mathrm{\Omega_\mathrm{O}}}{\partial v_\mathrm{i}} + \hat{v}_\mathrm{k} \frac{\partial v_\mathrm{k}}{\partial x_\mathrm{i}} - v_\mathrm{k} \frac{\partial \hat{v}_\mathrm{i}}{\partial x_\mathrm{k}} - 2 \nu \frac{\partial \hat{S}_\mathrm{ik}}{\partial x_\mathrm{k}} + \frac{\partial \hat{p} }{\partial x_\mathrm{i}} \right] \mathrm{d} \Omega,
\end{align}
Derivative in pressure direction:
\begin{align}
\delta_\mathrm{p} L \cdot \delta p &= \int_\mathrm{\Gamma} \frac{\partial j_\mathrm{\Gamma_\mathrm{O}}}{\partial p} \delta p \mathrm{d} \Gamma \\
& + \int_{\mathrm{\Gamma}_\mathrm{in}} \hat{p} \frac{\partial \delta p}{\partial n} \mathrm{d} \Gamma  \\
& + \int_{\mathrm{\Gamma}_\mathrm{out}} \hat{p} \frac{\partial \delta p}{\partial n} \mathrm{d} \Gamma \\
& + \int_{\mathrm{\Gamma}_\mathrm{wall}} \hat{p} \frac{\partial \delta p}{\partial n} \mathrm{d} \Gamma \\
& + \int_{\Omega} \frac{\partial j_\mathrm{\Omega_\mathrm{O}}}{\partial p} \delta p + \hat{v}_\mathrm{i}  \frac{\partial \delta p}{\partial x_\mathrm{i}} \frac{1}{\rho}  \mathrm{d} \Omega
\end{align}
can be rearranged to:
\begin{align}
\delta_\mathrm{p} L \cdot \delta p &= 
 \int_{\mathrm{\Gamma}_\mathrm{in}} \hat{p} \frac{\partial \delta p}{\partial n} \mathrm{d} \Gamma  \\
& + \int_{\mathrm{\Gamma}_\mathrm{out}} \hat{p} \frac{\partial \delta p}{\partial n} \mathrm{d} \Gamma \\
& + \int_{\mathrm{\Gamma}_\mathrm{wall}} \hat{p} \frac{\partial \delta p}{\partial n} \mathrm{d} \Gamma \\
& + \int_\mathrm{\Gamma} (\delta p) \left[\frac{\partial j_\mathrm{\Gamma_\mathrm{O}}}{\partial p} + \hat{v}_\mathrm{i} \frac{1}{\rho} n_\mathrm{i} \right] \mathrm{d} \Gamma \\
& + \int_{\Omega} (\delta p) \left[ \frac{\partial j_\mathrm{\Omega_\mathrm{O}}}{\partial p} -  \frac{\partial \hat{v}_\mathrm{i}}{\partial x_\mathrm{i}} \frac{1}{\rho} \right] \mathrm{d} \Omega.
\end{align}

\subsection{Adjoint Simplifaction}
Adjoint non-dimensional equations:
\begin{align}
\hat{R}_\mathrm{1}^*:&
- v_\mathrm{1}^* \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1} \hat{V}_\mathrm{1}}{L}
- v_\mathrm{2}^* \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{2} \hat{V}_\mathrm{1}}{\hat{\delta}}
+ \hat{v}_\mathrm{1}^* \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{\hat{V}_\mathrm{1} V_\mathrm{1}}{L}
+ \hat{v}_\mathrm{2}^* \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \frac{\hat{V}_\mathrm{2} V_\mathrm{2}}{L}
+ \frac{1}{L} \frac{\partial}{\partial x_\mathrm{1}^*} \left[ \hat{p}^* \hat{P} - \nu \left( \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{\hat{V}_\mathrm{1}}{L}  + \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{\hat{V}_\mathrm{1}}{L} \right) \right] \\
&+ \frac{1}{\hat{\delta}}\frac{\partial}{\partial x_\mathrm{2}^*} \left[ - \nu \left( \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{\hat{V}_\mathrm{1}}{\hat{\delta}}  + \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \frac{\hat{V}_\mathrm{2}}{L} \right) \right] + \frac{\partial j_\mathrm{\Omega_\mathrm{O}}^*}{\partial v_\mathrm{1}^*} \frac{J_\mathrm{v}}{\hat{V}_\mathrm{1}} = 0\\
\hat{R}_\mathrm{2}^*:&
- v_\mathrm{1}^* \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1} \hat{V}_\mathrm{2}}{L}
- v_\mathrm{2}^* \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{2} \hat{V}_\mathrm{2}}{\hat{\delta}}
+ \hat{v}_\mathrm{1}^* \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{\hat{V}_\mathrm{1} V_\mathrm{1}}{\delta}
+ \hat{v}_\mathrm{2}^* \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{\hat{V}_\mathrm{2} V_\mathrm{2}}{\delta}
+ \frac{1}{L}\frac{\partial}{\partial x_\mathrm{1}^*} \left[ - \nu \left( \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \frac{\hat{V}_\mathrm{2}}{L}  + \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{\hat{V}_\mathrm{1}}{\hat{\delta}} \right) \right] \\
&+ \frac{1}{\hat{\delta}} \frac{\partial}{\partial x_\mathrm{2}^*} \left[ \hat{p}^* \hat{P} - \nu \left( \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{\hat{V}_\mathrm{2}}{\hat{\delta}}  + \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*}\frac{\hat{V}_\mathrm{2}}{\hat{\delta}}  \right) \right] + \frac{\partial j_\mathrm{\Omega_\mathrm{O}}^*}{\partial v_\mathrm{2}^*} \frac{J_\mathrm{v}}{V_\mathrm{2}} = 0\\
\hat{Q}^*:&  -\frac{1}{\rho}\frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{\hat{V}_\mathrm{1}}{L} -\frac{1}{\rho}\frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{\hat{V}_\mathrm{2}}{\hat{\delta}} + \frac{\partial j_\mathrm{\Omega_\mathrm{O}}^*}{\partial p^*} \frac{J_\mathrm{p}}{P} = 0
\end{align}
Assuming $V_\mathrm{2} \propto V_\mathrm{1} \delta / L$ and $\hat{V}_\mathrm{2} \propto \hat{V}_\mathrm{1} \hat{\delta} / L + J_\mathrm{p} \hat{\delta} / P$:
\begin{align}
\hat{R}_\mathrm{1}^*:&
- v_\mathrm{1}^* \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1} \hat{V}_\mathrm{1}}{L}
- v_\mathrm{2}^* \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{1} \delta \hat{V}_\mathrm{1}}{\hat{\delta} L}
+ \hat{v}_\mathrm{1}^* \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{\hat{V}_\mathrm{1} V_\mathrm{1}}{L}
+ \hat{v}_\mathrm{2}^* \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \left[\frac{\hat{V}_\mathrm{1} \hat{\delta} V_\mathrm{1} \hat{\delta}}{L L L} + \frac{ J_\mathrm{p} \hat{\delta} V_\mathrm{1} \delta}{L L P} \right] \\
&+ \frac{1}{L} \frac{\partial}{\partial x_\mathrm{1}^*} \left[ \hat{p}^* \hat{P} - \nu \left( \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{\hat{V}_\mathrm{1}}{L}  + \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{\hat{V}_\mathrm{1}}{L} \right) \right]
+ \frac{1}{\hat{\delta}}\frac{\partial}{\partial x_\mathrm{2}^*} \left[ - \nu \left( \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{\hat{V}_\mathrm{1}}{\hat{\delta}}  + \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \left[ \frac{\hat{V}_\mathrm{1} \hat{\delta}}{L L} + \frac{J_\mathrm{p} \hat{\delta}}{L P}  \right] \right) \right] + \frac{\partial j_\mathrm{\Omega_\mathrm{O}}^*}{\partial v_\mathrm{1}^*} \frac{J_\mathrm{v}}{\hat{V}_\mathrm{1}} = 0\\
\hat{R}_\mathrm{2}^*:&
- v_\mathrm{1}^* \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \left[\frac{V_\mathrm{1} \hat{V}_\mathrm{1} \hat{\delta}}{L L} + \frac{V_\mathrm{1} J_\mathrm{p} \hat{\delta}}{L P} \right]
- v_\mathrm{2}^* \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \left[ \frac{V_\mathrm{1} \delta \hat{V}_\mathrm{1} \hat{\delta}}{\hat{\delta} L L} + \frac{V_\mathrm{1} \delta J_\mathrm{p} \hat{\delta}}{\hat{\delta} L P} \right]
+ \hat{v}_\mathrm{1}^* \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{\hat{V}_\mathrm{1} V_\mathrm{1}}{\delta}
+ \hat{v}_\mathrm{2}^* \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \left[ \frac{\hat{V}_\mathrm{1} \hat{\delta} V_\mathrm{1} \delta}{\delta L L} + \frac{J_\mathrm{p} \hat{\delta} V_\mathrm{1} \delta}{\delta L P} \right] \\
&+ \frac{1}{L}\frac{\partial}{\partial x_\mathrm{1}^*} \left[ - \nu \left( \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \left[ \frac{\hat{V}_\mathrm{1} \hat{\delta}}{L L} + \frac{ J \hat{\delta}}{L P} \right]  + \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{\hat{V}_\mathrm{1}}{\hat{\delta}} \right) \right]
+ \frac{1}{\hat{\delta}} \frac{\partial}{\partial x_\mathrm{2}^*} \left[ \hat{p}^* \hat{P} - \nu \left[ \frac{\hat{V}_\mathrm{1} \hat{\delta}}{\hat{\delta} L} + \frac{J_\mathrm{p} \hat{\delta}}{\hat{\delta} P} \right] \left( \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*} + \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \right) \right] + \frac{\partial j_\mathrm{\Omega_\mathrm{O}}^*}{\partial v_\mathrm{2}^*} \frac{J_\mathrm{v} L}{V_\mathrm{1} \delta} = 0\\
\hat{Q}^*:&  -\frac{1}{\rho}\frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{\hat{V}_\mathrm{1}}{L} -\frac{1}{\rho}\frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{\hat{V}_\mathrm{2}}{\hat{\delta}} + \frac{\partial j_\mathrm{\Omega_\mathrm{O}}^*}{\partial p^*} \frac{J_\mathrm{p}}{P} = 0
\end{align}
We end up with
\begin{align}
\hat{R}_\mathrm{1}^*:&
- v_\mathrm{1}^* \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*}
- v_\mathrm{2}^* \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{\delta}{\hat{\delta}}
+ \hat{v}_\mathrm{1}^* \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*}
+ \hat{v}_\mathrm{2}^* \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \left[\frac{\hat{\delta}^2}{L^2} + \frac{ J_\mathrm{p} \hat{\delta} \delta}{L \hat{V}_\mathrm{1} P} \right] \\
&+ \frac{\partial}{\partial x_\mathrm{1}^*} \left[ \hat{p}^* \frac{\hat{P}}{V_\mathrm{1} \hat{V}_\mathrm{1}} - \frac{\nu}{V_\mathrm{1} L} L \left( \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*} + \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \right) \right]
+ \frac{\partial}{\partial x_\mathrm{2}^*} \left[ - \frac{\nu}{V_\mathrm{1} L} \left( \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{L^2}{\hat{\delta}^2}  + \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \left[ 1 + \frac{L}{\hat{\delta}} \frac{J_\mathrm{p} \hat{\delta}}{\hat{V}_\mathrm{1} P} \right] \right) \right] + \frac{\partial j_\mathrm{\Omega_\mathrm{O}}^*}{\partial v_\mathrm{1}^*} \frac{J_\mathrm{v} L}{V_\mathrm{1} \hat{V}_\mathrm{1}^2} = 0\\
\hat{R}_\mathrm{2}^*:&
- v_\mathrm{1}^* \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \left[\frac{ \hat{\delta}}{ L} + \frac{ J_\mathrm{p} \hat{\delta}}{ \hat{V}_\mathrm{1} P} \right]
- v_\mathrm{2}^* \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \left[ \frac{\delta}{ L} + \frac{ \delta J_\mathrm{p} }{\hat{V}_\mathrm{1} P} \right]
+ \hat{v}_\mathrm{1}^* \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{L}{\delta}
+ \hat{v}_\mathrm{2}^* \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \left[ \frac{\hat{\delta}}{ L} + \frac{J_\mathrm{p} \hat{\delta} }{ \hat{V}_\mathrm{1} P} \right] \\
&+ \frac{\partial}{\partial x_\mathrm{1}^*} \left[ - \frac{\nu}{V_\mathrm{1} L} \left( \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \left[ \frac{\hat{\delta}}{L } + \frac{J_\mathrm{p} \hat{\delta}}{\hat{V}_\mathrm{1} P} \right]  + \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{\hat{V}_\mathrm{1}}{\hat{\delta}} \right) \right] \\
&+ \frac{\partial}{\partial x_\mathrm{2}^*} \left[ \hat{p}^* \frac{\hat{P}}{\hat{V}_\mathrm{1} V_\mathrm{1}} \frac{L}{\hat{\delta}} - \frac{\nu}{V_\mathrm{1} L} \left[ \frac{L}{\hat{\delta}} + \frac{J_\mathrm{p} L^2}{\hat{\delta} P \hat{V}_\mathrm{1}} \right] \left( \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*} + \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \right) \right] + \frac{\partial j_\mathrm{\Omega_\mathrm{O}}^*}{\partial v_\mathrm{2}^*} \frac{J_\mathrm{v} L^2}{V_\mathrm{1}^2 \hat{V}_\mathrm{1} \delta} = 0\\
\hat{Q}^*:&  -\frac{1}{\rho}\frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{\hat{V}_\mathrm{1}}{L} -\frac{1}{\rho}\frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \left[ \frac{\hat{V}_\mathrm{1} \hat{\delta}}{\hat{\delta} L} + \frac{J_\mathrm{p} \hat{\delta}}{\hat{\delta} P} \right] + \frac{\partial j_\mathrm{\Omega_\mathrm{O}}^*}{\partial p^*} \frac{J_\mathrm{p}}{P} = 0.
\end{align}
Interpreting this is really tough, which is why we set $J_\mathrm{p} = 0$:
\begin{align}
\hat{R}_\mathrm{1}^*:&
- v_\mathrm{1}^* \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*}
- v_\mathrm{2}^* \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{\delta}{\hat{\delta}}
+ \hat{v}_\mathrm{1}^* \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*}
+ \hat{v}_\mathrm{2}^* \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \frac{\hat{\delta}^2}{L^2} \\
&+ \frac{\partial}{\partial x_\mathrm{1}^*} \left[ \hat{p}^* \frac{\hat{P}}{V_\mathrm{1} \hat{V}_\mathrm{1}} - \frac{\nu}{V_\mathrm{1} L} L \left( \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*} + \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \right) \right]
+ \frac{\partial}{\partial x_\mathrm{2}^*} \left[ - \frac{\nu}{V_\mathrm{1} L} \left( \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{L^2}{\hat{\delta}^2}  + \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \right) \right] + \frac{\partial j_\mathrm{\Omega_\mathrm{O}}^*}{\partial v_\mathrm{1}^*} \frac{J_\mathrm{v} L}{V_\mathrm{1} \hat{V}_\mathrm{1}^2} = 0\\
\hat{R}_\mathrm{2}^*:&
- v_\mathrm{1}^* \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \frac{ \hat{\delta}}{ L} 
- v_\mathrm{2}^* \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{\delta}{ L} 
+ \hat{v}_\mathrm{1}^* \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{L}{\delta}
+ \hat{v}_\mathrm{2}^* \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{\hat{\delta}}{ L} \\
&+ \frac{\partial}{\partial x_\mathrm{1}^*} \left[ - \frac{\nu}{V_\mathrm{1} L} \left( \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \frac{\hat{\delta}}{L }  + \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{\hat{V}_\mathrm{1}}{\hat{\delta}} \right) \right] + \frac{\partial}{\partial x_\mathrm{2}^*} \left[ \hat{p}^* \frac{\hat{P}}{\hat{V}_\mathrm{1} V_\mathrm{1}} \frac{L}{\hat{\delta}} - \frac{\nu}{V_\mathrm{1} L} \frac{L}{\hat{\delta}} \left( \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*} + \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \right) \right] + \frac{\partial j_\mathrm{\Omega_\mathrm{O}}^*}{\partial v_\mathrm{2}^*} \frac{J_\mathrm{v} L^2}{V_\mathrm{1}^2 \hat{V}_\mathrm{1} \delta} = 0\\
\hat{Q}^*:&  - \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*} - \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*}  = 0.
\end{align}

\subsection{Adjoint Boundary Layer Equation}
\begin{align}
L &= \int_\mathrm{\Gamma_\mathrm{O}} j_\mathrm{\Gamma} \mathrm{d} \Gamma 
+ \int_{\mathrm{\Gamma}_\mathrm{wall}} \hat{v}_\mathrm{i} v_\mathrm{i}
+ \hat{p} \frac{\partial p}{\partial n} \mathrm{d} \Gamma \\
%& + \int_{\mathrm{ \partial \Omega}} \hat{v}_\mathrm{i} \left[ \frac{\partial v_\mathrm{i}}{\partial n} \right] + \hat{p} \frac{\partial p}{\partial n} + \hat{v_\mathrm{i}} \left[ v_\mathrm{i} - n_\mathrm{i} V_\mathrm{in} \right] + \hat{p} \frac{\partial p}{\partial n} \mathrm{d} \Gamma \\
& + \int_{\Omega} \hat{v}_\mathrm{1}  \left[ v_\mathrm{1} \frac{\partial v_\mathrm{1}}{\partial x_\mathrm{1}} + v_\mathrm{2} \frac{\partial v_\mathrm{1}}{\partial x_\mathrm{2}} + \frac{\partial p}{\partial x_\mathrm{1}} \frac{1}{\rho}  - \nu \frac{\partial^2 v_\mathrm{1}}{\partial {x_\mathrm{2}}^2} \right] \\
& \hspace{1cm} + \hat{v}_\mathrm{2} \left[  \frac{\partial p}{\partial x_\mathrm{2}} \frac{1}{\rho} \right]  + \hat{p} \left[ \frac{\partial v_\mathrm{1}}{\partial x_\mathrm{1}} + \frac{\partial v_\mathrm{2}}{\partial x_\mathrm{2}} \right] \mathrm{d} \Omega
\end{align}
Derivative in pressure direction:
\begin{align}
\delta_\mathrm{p} L \cdot \delta p
&= \int_\mathrm{\Gamma_\mathrm{O}} \frac{\partial j_\mathrm{\Gamma}}{\partial p} \delta p \mathrm{d} \Gamma 
+ \int_{\mathrm{\Gamma}_\mathrm{wall}} \hat{p} \frac{\partial (\delta p)}{\partial n} \mathrm{d} \Gamma \\
& + \int_{\Omega} \hat{v}_\mathrm{1}  \left[ \frac{\partial (\delta p)}{\partial x_\mathrm{1}} \frac{1}{\rho} \right]
+ \hat{v}_\mathrm{2} \left[ \frac{\partial (\delta p) }{\partial x_\mathrm{2}} \frac{1}{\rho} \right]  \mathrm{d} \Omega
\end{align}
can be rearranged to:
\begin{align}
\delta_\mathrm{p} L \cdot \delta p
&= \int_\mathrm{\Gamma_\mathrm{O}} \frac{\partial j_\mathrm{\Gamma}}{\partial p} \delta p \mathrm{d} \Gamma 
+ \int_{\mathrm{\Gamma}_\mathrm{wall}} \hat{p} \frac{\partial (\delta p)}{\partial n} \mathrm{d} \Gamma \\
&+ \int_{\Gamma} \delta p \left[ \hat{v}_\mathrm{1} n_\mathrm{1} \frac{1}{\rho} +\hat{v}_\mathrm{2} n_\mathrm{2} \frac{1}{\rho}  \right] \mathrm{d} \Gamma \&+ \int_{\Omega} \delta p  \left[ - \frac{\partial \hat{v}_\mathrm{1}}{\partial x_\mathrm{1}} \frac{1}{\rho} - \frac{\partial \hat{v}_\mathrm{2}}{\partial x_\mathrm{2}} \frac{1}{\rho} \right] \mathrm{d} \Omega.
\end{align}
Derivative in velocity direction:
\begin{align}
\delta_\mathrm{v_\mathrm{i}} L \cdot \delta v_\mathrm{i}  
= \delta_\mathrm{v_\mathrm{1}} L \cdot \delta v_\mathrm{1} 
+ \delta_\mathrm{v_\mathrm{2}} L \cdot \delta v_\mathrm{2} 
&= \int_\mathrm{\Gamma_\mathrm{O}} \frac{\partial j_\mathrm{\Gamma}}{\partial v_\mathrm{1}} \delta v_\mathrm{1} + \frac{\partial j_\mathrm{\Gamma}}{\partial v_\mathrm{2}} \delta v_\mathrm{2} \mathrm{d} \Gamma 
+ \int_{\mathrm{\Gamma}_\mathrm{wall}} \hat{v}_\mathrm{1} \delta v_\mathrm{1} + \hat{v}_\mathrm{2} \delta v_\mathrm{2}  \mathrm{d} \Gamma \\
& + \int_{\Omega} \hat{v}_\mathrm{1}  \left[ \delta v_\mathrm{1} \frac{\partial v_\mathrm{1}}{\partial x_\mathrm{1}} +  v_\mathrm{1} \frac{\partial (\delta v_\mathrm{1})}{\partial x_\mathrm{1}} + \delta v_\mathrm{2} \frac{\partial v_\mathrm{1}}{\partial x_\mathrm{2}} + v_\mathrm{2} \frac{\partial (\delta v_\mathrm{1})}{\partial x_\mathrm{2}}  - \nu \frac{\partial^2 (\delta v_\mathrm{1})}{\partial {x_\mathrm{2}}^2} \right] \\
& \hspace{1cm}  + \hat{p} \left[\frac{\partial (\delta v_\mathrm{1})}{\partial x_\mathrm{1}} + \frac{\partial (\delta v_\mathrm{2})}{\partial x_\mathrm{2}} \right] \mathrm{d} \Omega
\end{align}
can be rearranged to:
\begin{align}
\delta_\mathrm{v_\mathrm{i}} L \cdot \delta v_\mathrm{i}  
= \delta_\mathrm{v_\mathrm{1}} L \cdot \delta v_\mathrm{1} 
+ \delta_\mathrm{v_\mathrm{2}} L \cdot \delta v_\mathrm{2} 
&= \int_\mathrm{\Gamma_\mathrm{O}} \frac{\partial j_\mathrm{\Gamma}}{\partial v_\mathrm{1}} \delta v_\mathrm{1} + \frac{\partial j_\mathrm{\Gamma}}{\partial v_\mathrm{2}} \delta v_\mathrm{2} \mathrm{d} \Gamma 
+ \int_{\mathrm{\Gamma}_\mathrm{wall}} \hat{v}_\mathrm{1} \delta v_\mathrm{1} + \hat{v}_\mathrm{2} \delta v_\mathrm{2}  \mathrm{d} \Gamma \\
& + \int_{\Gamma} \delta v_\mathrm{1}  \left[ \hat{v}_\mathrm{1} \frac{\partial v_\mathrm{1}}{\partial x_\mathrm{1}} + \hat{v}_\mathrm{1} v_\mathrm{1} n_\mathrm{1} + \hat{v}_\mathrm{1} v_\mathrm{2} n_\mathrm{2} - \hat{p} n_\mathrm{2} + \nu \frac{\partial \hat{v}_\mathrm{1}}{\partial x_\mathrm{2}} n_\mathrm{2}  \right] 
- \nu \left( \hat{v}_\mathrm{1} \frac{\partial (\delta v_\mathrm{1})}{\partial x_\mathrm{2}} n_\mathrm{2} \right) \\
& \hspace{5mm} + \delta v_\mathrm{2} \left[- \hat{p} n_\mathrm{2} \right] \mathrm{d} \Gamma \\
& + \int_{\Omega} \delta v_\mathrm{1}  \left[ \hat{v}_\mathrm{1} \frac{\partial v_\mathrm{1}}{\partial x_\mathrm{1}} - \frac{ \partial \hat{v}_\mathrm{1} v_\mathrm{1}}{\partial x_\mathrm{1}} - \frac{\partial \hat{v}_\mathrm{1} v_\mathrm{2} }{\partial x_\mathrm{2}} - \nu \frac{\partial^2 (\delta \hat{v}_\mathrm{1})}{\partial {x_\mathrm{2}}^2} - \frac{\partial \hat{p}}{\partial x_\mathrm{1}} \right] \\
& \hspace{5mm}+ \delta v_\mathrm{2}  \left[ \hat{v}_\mathrm{1} \frac{\partial v_\mathrm{1}}{\partial x_\mathrm{2}} - \frac{\partial \hat{p}}{\partial x_\mathrm{2}} \right] \mathrm{d} \Omega
\end{align}

\subsection{Primal Blasius Equation}
The definition of $u = \partial \psi^* / \partial y$ and $v = - \partial \psi^* / \partial x$ by knowing $\psi := \psi(x, y, \eta^*) = \beta \, \sqrt{x} \, \, f^* (\eta^*)$ and $\eta^* := \eta^* (x, y) = \alpha \, y / \sqrt{x}$ yields:
\begin{itemize}
\item $u \rightarrow a b f^\prime$
\item $\partial u / \partial x \rightarrow - a b f^{\prime \prime} b y \frac{1}{2} x^{-3/2}$
\item $\partial u / \partial y \rightarrow a b f^{\prime \prime} b x^{-1/2}$
\item $\partial u^2 / \partial y^2 \rightarrow a b f^{\prime \prime \prime} b x^{-1/2} b x^{-1/2}$
\item $v \rightarrow - a \frac{1}{2} x^{-1/2} f - a x^{1/2} f^\prime y b \left(-\frac{1}{2}\right) x^{-3/2}$
\end{itemize}
for each term in the boundary layer equation. In the absence of pressure gradient this results in:
\begin{align}
u \frac{\partial u}{\partial x} 
+ v \frac{\partial u}{\partial y}
- \nu \frac{\partial^2 u}{\partial {y}^2} 
&= 0 \\
-a b f^\prime  a b f^{\prime \prime} b \frac{1}{2} y x^{-3/2}
+ \left( - a \frac{1}{2} x^{-1/2} f - a x^{1/2} f^\prime y b \left(-\frac{1}{2}\right) x^{-3/2} \right) a b f^{\prime \prime} b x^{-1/2}
- \nu a b f^{\prime \prime \prime} b x^{-1/2} b x^{-1/2}
&= 0 \\
-a^2 b^3 f^\prime  f^{\prime \prime} y x^{-3/2}
- \left( x^{-1/2} f - b x^{-1} f^\prime y \right) a^2 b^2 f^{\prime \prime} x^{-1/2}
- 2 \nu a b^3 f^{\prime \prime \prime} x^{-1}
&= 0 \\
- a^2 b^2 f f^{\prime \prime} x^{-1}
- 2 \nu a b^3 f^{\prime \prime \prime} x^{-1}
&= 0 \\
- f f^{\prime \prime}
- 2 \nu \frac{b}{a} f^{\prime \prime \prime}
&= 0
\end{align}

\subsection{Adjoint Blasius Equation}
The definition of $\hat{u} = \partial \hat{\psi}^* / \partial y$ and $\hat{v} = - \partial \hat{\psi}^* / \partial x$ by knowing $\hat{\psi} := \hat{\psi}(x, y, \hat{\eta}^*) = \beta \, \sqrt{1-x} \, \, \hat{f}^* (\hat{\eta}^*)$ and $\hat{\eta}^* := \hat{\eta}^* (x, y) = \alpha \, y / \sqrt{1-x}$ yields:
\begin{itemize}
\item $\hat{u} \rightarrow \hat{a} \hat{b} \hat{f}^\prime$
\item $\partial \hat{u} / \partial x \rightarrow \hat{a} \hat{b} \hat{f}^{\prime \prime} \hat{b} y \frac{1}{2} (1-x)^{-3/2}$
\item $\partial \hat{u} / \partial y \rightarrow \hat{a} \hat{b} \hat{f}^{\prime \prime} \hat{b} (1-x)^{-1/2}$
\item $\partial \hat{u}^2 / \partial y^2 \rightarrow \hat{a} \hat{b} \hat{f}^{\prime \prime \prime} \hat{b} (1-x)^{-1/2} \hat{b} (1-x)^{-1/2}$
%\item $v \rightarrow - a \frac{1}{2} x^{-1/2} f - a x^{1/2} f^\prime y b \left(-\frac{1}{2}\right) x^{-3/2}$
\end{itemize}
for each term in the boundary layer equation. In the absence of pressure gradient this results in:
\begin{align}
-u \frac{\partial \hat{u}}{\partial x} 
-v \frac{\partial \hat{u}}{\partial y}
+\hat{u} \frac{\partial u}{\partial x} 
- \nu \frac{\partial^2 \hat{u}}{\partial y^2} 
&= 0 \\
- a b f^\prime \hat{a} \hat{b} \hat{f}^{\prime \prime} \hat{b} y \frac{1}{2} (1-x)^{-3/2}
+ a \frac{1}{2} x^{-1/2} f + a x^{1/2} f^\prime y b \left(-\frac{1}{2}\right) x^{-3/2} \hat{a} \hat{b} \hat{f}^{\prime \prime} \hat{b} (1-x)^{-1/2} & \\
- \hat{a} \hat{b} \hat{f}^\prime a b f^{\prime \prime} b y \frac{1}{2} x^{-3/2}
- \hat{a} \hat{b} \hat{f}^{\prime \prime \prime} \hat{b} (1-x)^{-1/2} \hat{b} (1-x)^{-1/2}
&= 0 \\
- \frac{1}{2} a b \hat{a} \hat{b}^2 f^\prime \hat{f}^{\prime \prime} y (1-x)^{-3/2}
+ \left[ x^{-1/2} f - x^{1/2} f^\prime y b x^{-3/2} \right]  \frac{1}{2} a \hat{a} \hat{b} \hat{f}^{\prime \prime} \hat{b} (1-x)^{-1/2} & \\
- \frac{1}{2} a b^2 \hat{a} \hat{b} \hat{f}^\prime f^{\prime \prime} y x^{-3/2}
- \hat{a} \hat{b}^3 \hat{f}^{\prime \prime \prime} (1-x)^{-1}
&= 0 \\
- \frac{1}{2} a b \hat{a} \hat{b}^2 f^\prime \hat{f}^{\prime \prime} y (1-x)^{-3/2}
+ \frac{1}{2} a \hat{a} \hat{b}^2 x^{-1/2} f \hat{f}^{\prime \prime} (1-x)^{-1/2} 
- \frac{1}{2} a b \hat{a} \hat{b}^2  f^\prime y  x^{-1} \hat{f}^{\prime \prime} (1-x)^{-1/2} & \\
- \frac{1}{2} a b^2 \hat{a} \hat{b} \hat{f}^\prime f^{\prime \prime} y x^{-3/2}
- \hat{a} \hat{b}^3 \hat{f}^{\prime \prime \prime} (1-x)^{-1}
&= 0 \\
- \frac{1}{2} a b \hat{a} \hat{b}^2 f^\prime \hat{f}^{\prime \prime} y^3 (1-x)^{-3/2}
+ \frac{1}{2} a \hat{a} \hat{b}^2 x^{-1/2} f \hat{f}^{\prime \prime} y^2 (1-x)^{-1/2} 
- \frac{1}{2} a b \hat{a} \hat{b}^2  f^\prime y^3  x^{-1} \hat{f}^{\prime \prime} (1-x)^{-1/2} & \\
- \frac{1}{2} a b^2 \hat{a} \hat{b} \hat{f}^\prime f^{\prime \prime} y^3 x^{-3/2}
- \hat{a} \hat{b}^3 \hat{f}^{\prime \prime \prime} y^2 (1-x)^{-1}
&= 0 \\
- \frac{1}{2} a b \hat{a} \hat{b}^2 f^\prime \hat{f}^{\prime \prime} \hat{\eta}^3 / \hat{b}^3
+ \frac{1}{2} a \hat{a} \hat{b}^2 f \hat{f}^{\prime \prime} \eta / b \hat{\eta} / \hat{b}
- \frac{1}{2} a b \hat{a} \hat{b}^2  f^\prime \eta^2 / b^2 \hat{f}^{\prime \prime} \hat{\eta} / \hat{b} & \\
- \frac{1}{2} a b^2 \hat{a} \hat{b} \hat{f}^\prime f^{\prime \prime} \eta^3 / b^3
- \hat{a} \hat{b}^3 \hat{f}^{\prime \prime \prime} \hat{\eta}^2 / \hat{b}^2
&= 0 \\
- \frac{1}{2} a \hat{a} \frac{b}{\hat{b}} f^\prime \hat{f}^{\prime \prime} \hat{\eta}^3 
+ \frac{1}{2} a \hat{a} \frac{\hat{b}}{b} f \hat{f}^{\prime \prime} \eta \hat{\eta} 
- \frac{1}{2} a \hat{a} \frac{\hat{b}}{b}  f^\prime \eta^2 \hat{f}^{\prime \prime} \hat{\eta}  & \\
- \frac{1}{2} a \hat{a} \frac{\hat{b}}{b} \hat{f}^\prime f^{\prime \prime} \eta^3 
- \hat{a} \hat{b} \hat{f}^{\prime \prime \prime} \hat{\eta}^2
&= 0 \\
- \frac{b^2}{\hat{b}^2} f^\prime \hat{f}^{\prime \prime} \hat{\eta}^3 
+ f \hat{f}^{\prime \prime} \eta \hat{\eta} 
- f^\prime \eta^2 \hat{f}^{\prime \prime} \hat{\eta} 
- \hat{f}^\prime f^{\prime \prime} \eta^3 
- 2 \frac{b}{a} \hat{f}^{\prime \prime \prime} \hat{\eta}^2
&= 0
\end{align}

==> tex/field_equation_derivations.tex <==
\section{Field Equation Area}
\subsection{Primal Simplification}
Primal non-dimensional equations:
\begin{align}
R_\mathrm{1}^*:&  \hspace{3cm}  
v_\mathrm{1}^* \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1} V_\mathrm{1}}{L} 
+ v_\mathrm{2}^* \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{2}^*}\frac{V_\mathrm{2} V_\mathrm{1}}{\delta} 
+ \frac{1}{L}\frac{\partial}{\partial x_\mathrm{1}^*} \left[ \frac{p^*}{\rho} P - \nu \left( \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1}}{L} +  \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1}}{L} \right) \right] \nonumber \\
&\hspace{4cm} 
+ \frac{1}{\delta} \frac{\partial}{\partial x_\mathrm{2}^*} \left[ - \nu \left( \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{1}}{\delta} +  \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{2}}{L} \right) \right] = 0 \\
R_\mathrm{2}^*:&  \hspace{3cm} 
v_\mathrm{1}^* \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1} V_\mathrm{2}}{L} 
+ v_\mathrm{2}^* \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{2} V_\mathrm{2}}{\delta} 
+ \frac{1}{L} \frac{\partial}{\partial x_\mathrm{1}^*} \left[ - \nu \left( \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{2}}{L} +  \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{1}}{\delta} \right) \right] \nonumber \\
&\hspace{4cm} 
+ \frac{1}{\delta} \frac{\partial}{\partial x_\mathrm{2}^*} \left[ \frac{p^*}{\rho} P - \nu \left( \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{2}}{\delta} +  \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{2}}{\delta} \right) \right] = 0 \\
Q^*:& \hspace{4cm} 
-\frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1}}{L}
-\frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{2}}{\delta}
= 0.
\end{align}
Assuming $V_\mathrm{2} \propto V_\mathrm{1} \delta / L$:
\begin{align}
R_\mathrm{1}^*:&  \hspace{3cm}  
v_\mathrm{1}^* \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1} V_\mathrm{1}}{L} 
+ v_\mathrm{2}^* \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{2}^*}\frac{V_\mathrm{1} \delta V_\mathrm{1}}{\delta L} 
+ \frac{1}{L}\frac{\partial}{\partial x_\mathrm{1}^*} \left[ \frac{p^*}{\rho} P - \nu \left( \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1}}{L} +  \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1}}{L} \right) \right] \nonumber \\
&\hspace{4cm} 
+ \frac{1}{\delta} \frac{\partial}{\partial x_\mathrm{2}^*} \left[ - \nu \left( \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{1}}{\delta} +  \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1} \delta}{L L} \right) \right] = 0 \\
R_\mathrm{2}^*:&  \hspace{3cm} 
v_\mathrm{1}^* \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1} V_\mathrm{1} \delta}{L L} 
+ v_\mathrm{2}^* \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{1} \delta V_\mathrm{1} \delta}{\delta L L} 
+ \frac{1}{L} \frac{\partial}{\partial x_\mathrm{1}^*} \left[ - \nu \left( \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1} \delta}{L L} +  \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{1}}{\delta} \right) \right] \nonumber \\
&\hspace{4cm} 
+ \frac{1}{\delta} \frac{\partial}{\partial x_\mathrm{2}^*} \left[ \frac{p^*}{\rho} P - \nu \left( \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{1} \delta}{\delta L} +  \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{1} \delta}{\delta L} \right) \right] = 0 \\
Q^*:& \hspace{4cm} 
-\frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1}}{L}
-\frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{1} \delta}{\delta L}
= 0.
\end{align}
We end up with:
\begin{align}
R_\mathrm{1}^*:&  \hspace{3cm}  
v_\mathrm{1}^* \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*}
+ v_\mathrm{2}^* \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{2}^*}
+ \frac{\partial}{\partial x_\mathrm{1}^*} \left[ p^* \frac{P }{\rho V_\mathrm{1} V_\mathrm{1}} - \frac{\nu}{V_\mathrm{1} L} \left( \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*} +  \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \right) \right] \nonumber \\
&\hspace{4cm} 
+ \frac{\partial}{\partial x_\mathrm{2}^*} \left[- \frac{\nu}{V_\mathrm{1} L} \left( \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{L^2}{\delta^2} +  \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \right) \right] = 0 \\
R_\mathrm{2}^*:&  \hspace{3cm} 
v_\mathrm{1}^* \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{1}^*}
+ v_\mathrm{2}^* \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} 
+ \frac{\partial}{\partial x_\mathrm{1}^*} \left[- \frac{\nu}{V_\mathrm{1} L}  \left( \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{1}^*} +  \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{L^2}{\delta^2} \right) \right] \nonumber \\
&\hspace{4cm} 
+ \frac{\partial}{\partial x_\mathrm{2}^*} \left[ p^* \frac{P }{\rho V_\mathrm{1} V_\mathrm{1}} \frac{L^2}{\delta^2} - \frac{\nu}{V_\mathrm{1} L} \left( \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{L^2}{\delta^2} +  \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{L^2}{\delta^2} \right) \right] = 0 \\
Q^*:& \hspace{4cm} 
-\frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*} 
-\frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} 
= 0.
\end{align}

\subsection{Adjoint Derivation}
General Lagrangian reads:
\begin{align}
L &= \int_\mathrm{\Gamma} j_\mathrm{\Gamma_\mathrm{O}} \mathrm{d} \Gamma \\
& + \int_{\mathrm{\Gamma}_\mathrm{in}} \hat{v_\mathrm{i}} \left[ v_\mathrm{i} - n_\mathrm{i} v_\mathrm{i}^\mathrm{in} \right] \hat{p} \frac{\partial p}{\partial n} \mathrm{d} \Gamma  \\
& + \int_{\mathrm{\Gamma}_\mathrm{out}} \hat{v_\mathrm{i}} \left[ \frac{\partial v_\mathrm{i}}{\partial n} \right] + \hat{p} \frac{\partial p}{\partial n} \mathrm{d} \Gamma \\
& + \int_{\mathrm{\Gamma}_\mathrm{wall}} \hat{v_\mathrm{i}} v_\mathrm{i} + \hat{p} \frac{\partial p}{\partial n} \mathrm{d} \Gamma \\
& + \int_{\Omega} j_\mathrm{\Omega_\mathrm{O}} + \hat{v}_\mathrm{i} \left[ v_\mathrm{k} \frac{\partial v_\mathrm{i}}{\partial x_\mathrm{k}} + \frac{\partial}{\partial x_\mathrm{k}} \left[ \frac{p}{\rho} \delta_\mathrm{ik} - 2 \nu S_\mathrm{ik} \right] \right] - \hat{p} \frac{\partial v_\mathrm{i}}{\partial x_\mathrm{i}}\mathrm{d} \Omega.
\end{align}
Derivative in velocity direction:
\begin{align}
\delta_\mathrm{v_\mathrm{i}} L \cdot \delta v_\mathrm{i} &= \int_\mathrm{\Gamma} \frac{\partial j_\mathrm{\Gamma_\mathrm{O}}}{\partial v_\mathrm{i}} \delta v_\mathrm{i} \mathrm{d} \Gamma \\
& + \int_{\mathrm{\Gamma}_\mathrm{in}} \hat{v_\mathrm{i}} (\delta v_\mathrm{i}) \mathrm{d} \Gamma  \\
& + \int_{\mathrm{\Gamma}_\mathrm{out}} \hat{v_\mathrm{i}} \frac{\partial (\delta v_\mathrm{i})}{\partial n} \mathrm{d} \Gamma \\
& + \int_{\mathrm{\Gamma}_\mathrm{wall}} \hat{v_\mathrm{i}} (\delta v_\mathrm{i}) \mathrm{d} \Gamma \\
& + \int_{\Omega} \frac{\partial j_\mathrm{\Omega_\mathrm{O}}}{\partial v_\mathrm{i}} \delta v_\mathrm{i} + \hat{v}_\mathrm{i} \left[ \delta v_\mathrm{k} \frac{\partial v_\mathrm{i}}{\partial x_\mathrm{k}} + v_\mathrm{k} \frac{\partial (\delta v_\mathrm{i})}{\partial x_\mathrm{k}} - 2 \nu \frac{\partial (\delta S_\mathrm{ik})}{\partial x_\mathrm{k}} \right] - \hat{p} \frac{\partial (\delta v_\mathrm{i})}{\partial x_\mathrm{i}}\mathrm{d} \Omega,
\end{align}
can be rearranged to:
\begin{align}
\delta_\mathrm{v_\mathrm{i}} L \cdot \delta v_\mathrm{i} &= 
\int_{\mathrm{\Gamma}_\mathrm{in}} \hat{v_\mathrm{i}} (\delta v_\mathrm{i}) \mathrm{d} \Gamma  \\
& + \int_{\mathrm{\Gamma}_\mathrm{out}} \hat{v_\mathrm{i}} \frac{\partial (\delta v_\mathrm{i})}{\partial n} \mathrm{d} \Gamma \\
& + \int_{\mathrm{\Gamma}_\mathrm{wall}} \hat{v_\mathrm{i}} (\delta v_\mathrm{i}) \mathrm{d} \Gamma \\
& + \int_{\mathrm{\Gamma}}(\delta v_\mathrm{i}) \left[ \frac{\partial j_\mathrm{\Gamma_\mathrm{O}}}{\partial v_\mathrm{i}} + v_\mathrm{k} \hat{v}_\mathrm{i} n_\mathrm{k} + 2 \nu \hat{S}_\mathrm{ik}n_\mathrm{k} - \hat{p} n_\mathrm{i} \right] - (\delta S_\mathrm{ik}) \hat{v}_\mathrm{i} \nu   \mathrm{d} \Gamma \\
& + \int_{\Omega} \delta v_\mathrm{i} \left[ \frac{\partial j_\mathrm{\Omega_\mathrm{O}}}{\partial v_\mathrm{i}} + \hat{v}_\mathrm{k} \frac{\partial v_\mathrm{k}}{\partial x_\mathrm{i}} - v_\mathrm{k} \frac{\partial \hat{v}_\mathrm{i}}{\partial x_\mathrm{k}} - 2 \nu \frac{\partial \hat{S}_\mathrm{ik}}{\partial x_\mathrm{k}} + \frac{\partial \hat{p} }{\partial x_\mathrm{i}} \right] \mathrm{d} \Omega,
\end{align}
Derivative in pressure direction:
\begin{align}
\delta_\mathrm{p} L \cdot \delta p &= \int_\mathrm{\Gamma} \frac{\partial j_\mathrm{\Gamma_\mathrm{O}}}{\partial p} \delta p \mathrm{d} \Gamma \\
& + \int_{\mathrm{\Gamma}_\mathrm{in}} \hat{p} \frac{\partial \delta p}{\partial n} \mathrm{d} \Gamma  \\
& + \int_{\mathrm{\Gamma}_\mathrm{out}} \hat{p} \frac{\partial \delta p}{\partial n} \mathrm{d} \Gamma \\
& + \int_{\mathrm{\Gamma}_\mathrm{wall}} \hat{p} \frac{\partial \delta p}{\partial n} \mathrm{d} \Gamma \\
& + \int_{\Omega} \frac{\partial j_\mathrm{\Omega_\mathrm{O}}}{\partial p} \delta p + \hat{v}_\mathrm{i}  \frac{\partial \delta p}{\partial x_\mathrm{i}} \frac{1}{\rho}  \mathrm{d} \Omega
\end{align}
can be rearranged to:
\begin{align}
\delta_\mathrm{p} L \cdot \delta p &= 
 \int_{\mathrm{\Gamma}_\mathrm{in}} \hat{p} \frac{\partial \delta p}{\partial n} \mathrm{d} \Gamma  \\
& + \int_{\mathrm{\Gamma}_\mathrm{out}} \hat{p} \frac{\partial \delta p}{\partial n} \mathrm{d} \Gamma \\
& + \int_{\mathrm{\Gamma}_\mathrm{wall}} \hat{p} \frac{\partial \delta p}{\partial n} \mathrm{d} \Gamma \\
& + \int_\mathrm{\Gamma} (\delta p) \left[\frac{\partial j_\mathrm{\Gamma_\mathrm{O}}}{\partial p} + \hat{v}_\mathrm{i} \frac{1}{\rho} n_\mathrm{i} \right] \mathrm{d} \Gamma \\
& + \int_{\Omega} (\delta p) \left[ \frac{\partial j_\mathrm{\Omega_\mathrm{O}}}{\partial p} -  \frac{\partial \hat{v}_\mathrm{i}}{\partial x_\mathrm{i}} \frac{1}{\rho} \right] \mathrm{d} \Omega.
\end{align}

\subsection{Adjoint Simplifaction}
Adjoint non-dimensional equations:
\begin{align}
\hat{R}_\mathrm{1}^*:&
- v_\mathrm{1}^* \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1} \hat{V}_\mathrm{1}}{L}
- v_\mathrm{2}^* \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{2} \hat{V}_\mathrm{1}}{\hat{\delta}}
+ \hat{v}_\mathrm{1}^* \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{\hat{V}_\mathrm{1} V_\mathrm{1}}{L}
+ \hat{v}_\mathrm{2}^* \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \frac{\hat{V}_\mathrm{2} V_\mathrm{2}}{L}
+ \frac{1}{L} \frac{\partial}{\partial x_\mathrm{1}^*} \left[ \hat{p}^* \hat{P} - \nu \left( \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{\hat{V}_\mathrm{1}}{L}  + \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{\hat{V}_\mathrm{1}}{L} \right) \right] \\
&+ \frac{1}{\hat{\delta}}\frac{\partial}{\partial x_\mathrm{2}^*} \left[ - \nu \left( \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{\hat{V}_\mathrm{1}}{\hat{\delta}}  + \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \frac{\hat{V}_\mathrm{2}}{L} \right) \right] + \frac{\partial j_\mathrm{\Omega_\mathrm{O}}^*}{\partial v_\mathrm{1}^*} \frac{J_\mathrm{v}}{\hat{V}_\mathrm{1}} = 0\\
\hat{R}_\mathrm{2}^*:&
- v_\mathrm{1}^* \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1} \hat{V}_\mathrm{2}}{L}
- v_\mathrm{2}^* \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{2} \hat{V}_\mathrm{2}}{\hat{\delta}}
+ \hat{v}_\mathrm{1}^* \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{\hat{V}_\mathrm{1} V_\mathrm{1}}{\delta}
+ \hat{v}_\mathrm{2}^* \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{\hat{V}_\mathrm{2} V_\mathrm{2}}{\delta}
+ \frac{1}{L}\frac{\partial}{\partial x_\mathrm{1}^*} \left[ - \nu \left( \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \frac{\hat{V}_\mathrm{2}}{L}  + \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{\hat{V}_\mathrm{1}}{\hat{\delta}} \right) \right] \\
&+ \frac{1}{\hat{\delta}} \frac{\partial}{\partial x_\mathrm{2}^*} \left[ \hat{p}^* \hat{P} - \nu \left( \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{\hat{V}_\mathrm{2}}{\hat{\delta}}  + \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*}\frac{\hat{V}_\mathrm{2}}{\hat{\delta}}  \right) \right] + \frac{\partial j_\mathrm{\Omega_\mathrm{O}}^*}{\partial v_\mathrm{2}^*} \frac{J_\mathrm{v}}{V_\mathrm{2}} = 0\\
\hat{Q}^*:&  -\frac{1}{\rho}\frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{\hat{V}_\mathrm{1}}{L} -\frac{1}{\rho}\frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{\hat{V}_\mathrm{2}}{\hat{\delta}} + \frac{\partial j_\mathrm{\Omega_\mathrm{O}}^*}{\partial p^*} \frac{J_\mathrm{p}}{P} = 0
\end{align}
Assuming $V_\mathrm{2} \propto V_\mathrm{1} \delta / L$ and $\hat{V}_\mathrm{2} \propto \hat{V}_\mathrm{1} \hat{\delta} / L + J_\mathrm{p} \hat{\delta} / P$:
\begin{align}
\hat{R}_\mathrm{1}^*:&
- v_\mathrm{1}^* \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{V_\mathrm{1} \hat{V}_\mathrm{1}}{L}
- v_\mathrm{2}^* \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{V_\mathrm{1} \delta \hat{V}_\mathrm{1}}{\hat{\delta} L}
+ \hat{v}_\mathrm{1}^* \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{\hat{V}_\mathrm{1} V_\mathrm{1}}{L}
+ \hat{v}_\mathrm{2}^* \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \left[\frac{\hat{V}_\mathrm{1} \hat{\delta} V_\mathrm{1} \hat{\delta}}{L L L} + \frac{ J_\mathrm{p} \hat{\delta} V_\mathrm{1} \delta}{L L P} \right] \\
&+ \frac{1}{L} \frac{\partial}{\partial x_\mathrm{1}^*} \left[ \hat{p}^* \hat{P} - \nu \left( \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{\hat{V}_\mathrm{1}}{L}  + \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{\hat{V}_\mathrm{1}}{L} \right) \right]
+ \frac{1}{\hat{\delta}}\frac{\partial}{\partial x_\mathrm{2}^*} \left[ - \nu \left( \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{\hat{V}_\mathrm{1}}{\hat{\delta}}  + \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \left[ \frac{\hat{V}_\mathrm{1} \hat{\delta}}{L L} + \frac{J_\mathrm{p} \hat{\delta}}{L P}  \right] \right) \right] + \frac{\partial j_\mathrm{\Omega_\mathrm{O}}^*}{\partial v_\mathrm{1}^*} \frac{J_\mathrm{v}}{\hat{V}_\mathrm{1}} = 0\\
\hat{R}_\mathrm{2}^*:&
- v_\mathrm{1}^* \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \left[\frac{V_\mathrm{1} \hat{V}_\mathrm{1} \hat{\delta}}{L L} + \frac{V_\mathrm{1} J_\mathrm{p} \hat{\delta}}{L P} \right]
- v_\mathrm{2}^* \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \left[ \frac{V_\mathrm{1} \delta \hat{V}_\mathrm{1} \hat{\delta}}{\hat{\delta} L L} + \frac{V_\mathrm{1} \delta J_\mathrm{p} \hat{\delta}}{\hat{\delta} L P} \right]
+ \hat{v}_\mathrm{1}^* \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{\hat{V}_\mathrm{1} V_\mathrm{1}}{\delta}
+ \hat{v}_\mathrm{2}^* \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \left[ \frac{\hat{V}_\mathrm{1} \hat{\delta} V_\mathrm{1} \delta}{\delta L L} + \frac{J_\mathrm{p} \hat{\delta} V_\mathrm{1} \delta}{\delta L P} \right] \\
&+ \frac{1}{L}\frac{\partial}{\partial x_\mathrm{1}^*} \left[ - \nu \left( \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \left[ \frac{\hat{V}_\mathrm{1} \hat{\delta}}{L L} + \frac{ J \hat{\delta}}{L P} \right]  + \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{\hat{V}_\mathrm{1}}{\hat{\delta}} \right) \right]
+ \frac{1}{\hat{\delta}} \frac{\partial}{\partial x_\mathrm{2}^*} \left[ \hat{p}^* \hat{P} - \nu \left[ \frac{\hat{V}_\mathrm{1} \hat{\delta}}{\hat{\delta} L} + \frac{J_\mathrm{p} \hat{\delta}}{\hat{\delta} P} \right] \left( \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*} + \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \right) \right] + \frac{\partial j_\mathrm{\Omega_\mathrm{O}}^*}{\partial v_\mathrm{2}^*} \frac{J_\mathrm{v} L}{V_\mathrm{1} \delta} = 0\\
\hat{Q}^*:&  -\frac{1}{\rho}\frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{\hat{V}_\mathrm{1}}{L} -\frac{1}{\rho}\frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{\hat{V}_\mathrm{2}}{\hat{\delta}} + \frac{\partial j_\mathrm{\Omega_\mathrm{O}}^*}{\partial p^*} \frac{J_\mathrm{p}}{P} = 0
\end{align}
We end up with
\begin{align}
\hat{R}_\mathrm{1}^*:&
- v_\mathrm{1}^* \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*}
- v_\mathrm{2}^* \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{\delta}{\hat{\delta}}
+ \hat{v}_\mathrm{1}^* \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*}
+ \hat{v}_\mathrm{2}^* \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \left[\frac{\hat{\delta}^2}{L^2} + \frac{ J_\mathrm{p} \hat{\delta} \delta}{L \hat{V}_\mathrm{1} P} \right] \\
&+ \frac{\partial}{\partial x_\mathrm{1}^*} \left[ \hat{p}^* \frac{\hat{P}}{V_\mathrm{1} \hat{V}_\mathrm{1}} - \frac{\nu}{V_\mathrm{1} L} L \left( \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*} + \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \right) \right]
+ \frac{\partial}{\partial x_\mathrm{2}^*} \left[ - \frac{\nu}{V_\mathrm{1} L} \left( \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{L^2}{\hat{\delta}^2}  + \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \left[ 1 + \frac{L}{\hat{\delta}} \frac{J_\mathrm{p} \hat{\delta}}{\hat{V}_\mathrm{1} P} \right] \right) \right] + \frac{\partial j_\mathrm{\Omega_\mathrm{O}}^*}{\partial v_\mathrm{1}^*} \frac{J_\mathrm{v} L}{V_\mathrm{1} \hat{V}_\mathrm{1}^2} = 0\\
\hat{R}_\mathrm{2}^*:&
- v_\mathrm{1}^* \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \left[\frac{ \hat{\delta}}{ L} + \frac{ J_\mathrm{p} \hat{\delta}}{ \hat{V}_\mathrm{1} P} \right]
- v_\mathrm{2}^* \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \left[ \frac{\delta}{ L} + \frac{ \delta J_\mathrm{p} }{\hat{V}_\mathrm{1} P} \right]
+ \hat{v}_\mathrm{1}^* \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{L}{\delta}
+ \hat{v}_\mathrm{2}^* \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \left[ \frac{\hat{\delta}}{ L} + \frac{J_\mathrm{p} \hat{\delta} }{ \hat{V}_\mathrm{1} P} \right] \\
&+ \frac{\partial}{\partial x_\mathrm{1}^*} \left[ - \frac{\nu}{V_\mathrm{1} L} \left( \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \left[ \frac{\hat{\delta}}{L } + \frac{J_\mathrm{p} \hat{\delta}}{\hat{V}_\mathrm{1} P} \right]  + \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{\hat{V}_\mathrm{1}}{\hat{\delta}} \right) \right] \\
&+ \frac{\partial}{\partial x_\mathrm{2}^*} \left[ \hat{p}^* \frac{\hat{P}}{\hat{V}_\mathrm{1} V_\mathrm{1}} \frac{L}{\hat{\delta}} - \frac{\nu}{V_\mathrm{1} L} \left[ \frac{L}{\hat{\delta}} + \frac{J_\mathrm{p} L^2}{\hat{\delta} P \hat{V}_\mathrm{1}} \right] \left( \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*} + \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \right) \right] + \frac{\partial j_\mathrm{\Omega_\mathrm{O}}^*}{\partial v_\mathrm{2}^*} \frac{J_\mathrm{v} L^2}{V_\mathrm{1}^2 \hat{V}_\mathrm{1} \delta} = 0\\
\hat{Q}^*:&  -\frac{1}{\rho}\frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \frac{\hat{V}_\mathrm{1}}{L} -\frac{1}{\rho}\frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \left[ \frac{\hat{V}_\mathrm{1} \hat{\delta}}{\hat{\delta} L} + \frac{J_\mathrm{p} \hat{\delta}}{\hat{\delta} P} \right] + \frac{\partial j_\mathrm{\Omega_\mathrm{O}}^*}{\partial p^*} \frac{J_\mathrm{p}}{P} = 0.
\end{align}
Interpreting this is really tough, which is why we set $J_\mathrm{p} = 0$:
\begin{align}
\hat{R}_\mathrm{1}^*:&
- v_\mathrm{1}^* \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*}
- v_\mathrm{2}^* \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{\delta}{\hat{\delta}}
+ \hat{v}_\mathrm{1}^* \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{1}^*}
+ \hat{v}_\mathrm{2}^* \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \frac{\hat{\delta}^2}{L^2} \\
&+ \frac{\partial}{\partial x_\mathrm{1}^*} \left[ \hat{p}^* \frac{\hat{P}}{V_\mathrm{1} \hat{V}_\mathrm{1}} - \frac{\nu}{V_\mathrm{1} L} L \left( \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*} + \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*} \right) \right]
+ \frac{\partial}{\partial x_\mathrm{2}^*} \left[ - \frac{\nu}{V_\mathrm{1} L} \left( \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{L^2}{\hat{\delta}^2}  + \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \right) \right] + \frac{\partial j_\mathrm{\Omega_\mathrm{O}}^*}{\partial v_\mathrm{1}^*} \frac{J_\mathrm{v} L}{V_\mathrm{1} \hat{V}_\mathrm{1}^2} = 0\\
\hat{R}_\mathrm{2}^*:&
- v_\mathrm{1}^* \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \frac{ \hat{\delta}}{ L} 
- v_\mathrm{2}^* \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{\delta}{ L} 
+ \hat{v}_\mathrm{1}^* \frac{\partial v_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{L}{\delta}
+ \hat{v}_\mathrm{2}^* \frac{\partial v_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \frac{\hat{\delta}}{ L} \\
&+ \frac{\partial}{\partial x_\mathrm{1}^*} \left[ - \frac{\nu}{V_\mathrm{1} L} \left( \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{1}^*} \frac{\hat{\delta}}{L }  + \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{2}^*} \frac{\hat{V}_\mathrm{1}}{\hat{\delta}} \right) \right] + \frac{\partial}{\partial x_\mathrm{2}^*} \left[ \hat{p}^* \frac{\hat{P}}{\hat{V}_\mathrm{1} V_\mathrm{1}} \frac{L}{\hat{\delta}} - \frac{\nu}{V_\mathrm{1} L} \frac{L}{\hat{\delta}} \left( \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*} + \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*} \right) \right] + \frac{\partial j_\mathrm{\Omega_\mathrm{O}}^*}{\partial v_\mathrm{2}^*} \frac{J_\mathrm{v} L^2}{V_\mathrm{1}^2 \hat{V}_\mathrm{1} \delta} = 0\\
\hat{Q}^*:&  - \frac{\partial \hat{v}_\mathrm{1}^*}{\partial x_\mathrm{1}^*} - \frac{\partial \hat{v}_\mathrm{2}^*}{\partial x_\mathrm{2}^*}  = 0.
\end{align}

\subsection{Adjoint Boundary Layer Equation}
\begin{align}
L &= \int_\mathrm{\Gamma_\mathrm{O}} j_\mathrm{\Gamma} \mathrm{d} \Gamma 
+ \int_{\mathrm{\Gamma}_\mathrm{wall}} \hat{v}_\mathrm{i} v_\mathrm{i}
+ \hat{p} \frac{\partial p}{\partial n} \mathrm{d} \Gamma \\
%& + \int_{\mathrm{ \partial \Omega}} \hat{v}_\mathrm{i} \left[ \frac{\partial v_\mathrm{i}}{\partial n} \right] + \hat{p} \frac{\partial p}{\partial n} + \hat{v_\mathrm{i}} \left[ v_\mathrm{i} - n_\mathrm{i} V_\mathrm{in} \right] + \hat{p} \frac{\partial p}{\partial n} \mathrm{d} \Gamma \\
& + \int_{\Omega} \hat{v}_\mathrm{1}  \left[ v_\mathrm{1} \frac{\partial v_\mathrm{1}}{\partial x_\mathrm{1}} + v_\mathrm{2} \frac{\partial v_\mathrm{1}}{\partial x_\mathrm{2}} + \frac{\partial p}{\partial x_\mathrm{1}} \frac{1}{\rho}  - \nu \frac{\partial^2 v_\mathrm{1}}{\partial {x_\mathrm{2}}^2} \right] \\
& \hspace{1cm} + \hat{v}_\mathrm{2} \left[  \frac{\partial p}{\partial x_\mathrm{2}} \frac{1}{\rho} \right]  + \hat{p} \left[ \frac{\partial v_\mathrm{1}}{\partial x_\mathrm{1}} + \frac{\partial v_\mathrm{2}}{\partial x_\mathrm{2}} \right] \mathrm{d} \Omega
\end{align}
Derivative in pressure direction:
\begin{align}
\delta_\mathrm{p} L \cdot \delta p
&= \int_\mathrm{\Gamma_\mathrm{O}} \frac{\partial j_\mathrm{\Gamma}}{\partial p} \delta p \mathrm{d} \Gamma 
+ \int_{\mathrm{\Gamma}_\mathrm{wall}} \hat{p} \frac{\partial (\delta p)}{\partial n} \mathrm{d} \Gamma \\
& + \int_{\Omega} \hat{v}_\mathrm{1}  \left[ \frac{\partial (\delta p)}{\partial x_\mathrm{1}} \frac{1}{\rho} \right]
+ \hat{v}_\mathrm{2} \left[ \frac{\partial (\delta p) }{\partial x_\mathrm{2}} \frac{1}{\rho} \right]  \mathrm{d} \Omega
\end{align}
can be rearranged to:
\begin{align}
\delta_\mathrm{p} L \cdot \delta p
&= \int_\mathrm{\Gamma_\mathrm{O}} \frac{\partial j_\mathrm{\Gamma}}{\partial p} \delta p \mathrm{d} \Gamma 
+ \int_{\mathrm{\Gamma}_\mathrm{wall}} \hat{p} \frac{\partial (\delta p)}{\partial n} \mathrm{d} \Gamma \\
&+ \int_{\Gamma} \delta p \left[ \hat{v}_\mathrm{1} n_\mathrm{1} \frac{1}{\rho} +\hat{v}_\mathrm{2} n_\mathrm{2} \frac{1}{\rho}  \right] \mathrm{d} \Gamma \&+ \int_{\Omega} \delta p  \left[ - \frac{\partial \hat{v}_\mathrm{1}}{\partial x_\mathrm{1}} \frac{1}{\rho} - \frac{\partial \hat{v}_\mathrm{2}}{\partial x_\mathrm{2}} \frac{1}{\rho} \right] \mathrm{d} \Omega.
\end{align}
Derivative in velocity direction:
\begin{align}
\delta_\mathrm{v_\mathrm{i}} L \cdot \delta v_\mathrm{i}  
= \delta_\mathrm{v_\mathrm{1}} L \cdot \delta v_\mathrm{1} 
+ \delta_\mathrm{v_\mathrm{2}} L \cdot \delta v_\mathrm{2} 
&= \int_\mathrm{\Gamma_\mathrm{O}} \frac{\partial j_\mathrm{\Gamma}}{\partial v_\mathrm{1}} \delta v_\mathrm{1} + \frac{\partial j_\mathrm{\Gamma}}{\partial v_\mathrm{2}} \delta v_\mathrm{2} \mathrm{d} \Gamma 
+ \int_{\mathrm{\Gamma}_\mathrm{wall}} \hat{v}_\mathrm{1} \delta v_\mathrm{1} + \hat{v}_\mathrm{2} \delta v_\mathrm{2}  \mathrm{d} \Gamma \\
& + \int_{\Omega} \hat{v}_\mathrm{1}  \left[ \delta v_\mathrm{1} \frac{\partial v_\mathrm{1}}{\partial x_\mathrm{1}} +  v_\mathrm{1} \frac{\partial (\delta v_\mathrm{1})}{\partial x_\mathrm{1}} + \delta v_\mathrm{2} \frac{\partial v_\mathrm{1}}{\partial x_\mathrm{2}} + v_\mathrm{2} \frac{\partial (\delta v_\mathrm{1})}{\partial x_\mathrm{2}}  - \nu \frac{\partial^2 (\delta v_\mathrm{1})}{\partial {x_\mathrm{2}}^2} \right] \\
& \hspace{1cm}  + \hat{p} \left[\frac{\partial (\delta v_\mathrm{1})}{\partial x_\mathrm{1}} + \frac{\partial (\delta v_\mathrm{2})}{\partial x_\mathrm{2}} \right] \mathrm{d} \Omega
\end{align}
can be rearranged to:
\begin{align}
\delta_\mathrm{v_\mathrm{i}} L \cdot \delta v_\mathrm{i}  
= \delta_\mathrm{v_\mathrm{1}} L \cdot \delta v_\mathrm{1} 
+ \delta_\mathrm{v_\mathrm{2}} L \cdot \delta v_\mathrm{2} 
&= \int_\mathrm{\Gamma_\mathrm{O}} \frac{\partial j_\mathrm{\Gamma}}{\partial v_\mathrm{1}} \delta v_\mathrm{1} + \frac{\partial j_\mathrm{\Gamma}}{\partial v_\mathrm{2}} \delta v_\mathrm{2} \mathrm{d} \Gamma 
+ \int_{\mathrm{\Gamma}_\mathrm{wall}} \hat{v}_\mathrm{1} \delta v_\mathrm{1} + \hat{v}_\mathrm{2} \delta v_\mathrm{2}  \mathrm{d} \Gamma \\
& + \int_{\Gamma} \delta v_\mathrm{1}  \left[ \hat{v}_\mathrm{1} \frac{\partial v_\mathrm{1}}{\partial x_\mathrm{1}} + \hat{v}_\mathrm{1} v_\mathrm{1} n_\mathrm{1} + \hat{v}_\mathrm{1} v_\mathrm{2} n_\mathrm{2} - \hat{p} n_\mathrm{2} + \nu \frac{\partial \hat{v}_\mathrm{1}}{\partial x_\mathrm{2}} n_\mathrm{2}  \right] 
- \nu \left( \hat{v}_\mathrm{1} \frac{\partial (\delta v_\mathrm{1})}{\partial x_\mathrm{2}} n_\mathrm{2} \right) \\
& \hspace{5mm} + \delta v_\mathrm{2} \left[- \hat{p} n_\mathrm{2} \right] \mathrm{d} \Gamma \\
& + \int_{\Omega} \delta v_\mathrm{1}  \left[ \hat{v}_\mathrm{1} \frac{\partial v_\mathrm{1}}{\partial x_\mathrm{1}} - \frac{ \partial \hat{v}_\mathrm{1} v_\mathrm{1}}{\partial x_\mathrm{1}} - \frac{\partial \hat{v}_\mathrm{1} v_\mathrm{2} }{\partial x_\mathrm{2}} - \nu \frac{\partial^2 (\delta \hat{v}_\mathrm{1})}{\partial {x_\mathrm{2}}^2} - \frac{\partial \hat{p}}{\partial x_\mathrm{1}} \right] \\
& \hspace{5mm}+ \delta v_\mathrm{2}  \left[ \hat{v}_\mathrm{1} \frac{\partial v_\mathrm{1}}{\partial x_\mathrm{2}} - \frac{\partial \hat{p}}{\partial x_\mathrm{2}} \right] \mathrm{d} \Omega
\end{align}
